Towards Automatic Support of Software Model Evolution with Large Language~Models

Modeling structure and behavior of software systems plays a crucial role, in various areas of software engineering. As with other software engineering artifacts, software models are subject to evolution. Supporting modelers in evolving models by model completion facilities and providing high-level edit operations such as frequently occurring editing patterns is still an open problem. Recently, large language models (i.e., generative neural networks) have garnered significant attention in various research areas, including software engineering. In this paper, we explore the potential of large language models in supporting the evolution of software models in software engineering. We propose an approach that utilizes large language models for model completion and discovering editing patterns in model histories of software systems. Through controlled experiments using simulated model repositories, we conduct an evaluation of the potential of large language models for these two tasks. We have found that large language models are indeed a promising technology for supporting software model evolution, and that it is worth investigating further in the area of software model evolution.

==> Content/4_1_generation_algo.tex <==

% \newcommand{\pluseq}{\mathrel{+}=}

% \begin{algorithm}
% \DontPrintSemicolon
% \small
% \SetCommentSty{\small}

% \SetKwFunction{generateCandidates}{generateCandidates}
% \SetKwFunction{checkCorrectSCG}{checkCorrectSCG}
% \SetKwFunction{sampleEdges}{sampleEdges}
% \SetKwFunction{checkMetaModel}{checkMetaModel}
% \SetKwFunction{complete}{complete}
% \SetKwFunction{prune}{prune}
% \SetKwFunction{size}{size}

% \SetKwData{lm}{$\mathcal{L}$}
% \SetKwData{mm}{$\mathcal{TM}$}

% \SetKwData{extendedEOs}{ext}
% \SetKwData{incompleteEOs}{incomplete}
% \SetKwData{completeEOs}{complete}

% \SetKwData{extendedEO}{$\tilde\varepsilon$}
% \SetKwData{eo}{op}

% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}

% \Input{$\varepsilon$ - given context serialization\\
% \lm - fine-tuned language model\\
% \mm - metamodel}
% \Output{$[\varepsilon_1,\dots,\varepsilon_n]$ - list of candidates}

% \BlankLine

% \incompleteEOs $\gets$ [$\varepsilon$]\tcc*{set of incomplete edit operations} 
% \completeEOs $\gets$ [] \tcc*{set of complete edit operations} 
% \While{\size{\incompleteEOs} $>0$}{       
% \extendedEOs $\gets$ []\tcc*{set of extended edit operations} 
% \ForEach{\eo $\in$ \incompleteEOs}{
% \extendedEOs $\pluseq$ \sampleEdges{\lm, \eo}\;
% \extendedEOs $\gets$ \checkCorrectSCG{\extendedEOs}\;
% \extendedEOs $\gets$ \checkMetaModel{\mm, \extendedEOs}\;
% \extendedEOs $\gets$ \prune{\extendedEOs, \completeEOs}\;
% \incompleteEOs $\gets$ []\;
% \ForEach{\extendedEO \in \extendedEOs}{
% \eIf{\complete{\extendedEO}}
% {\completeEOs $\pluseq$ \extendedEO \;}
% {\incompleteEOs $\pluseq$ \extendedEO \;}
% }
% }      
% }
% \Return{\completeEOs}

% \caption{Pseudocode for the candidate generation.\label{lst:candidateGeneration}}
% \end{algorithm}



% \begin{algorithm}
% \LinesNumbered
% \SetAlgoLined
% \small
% \SetCommentSty{\small}

% \SetKw{function}{Function}
% \SetKwFunction{generateCandidates}{generateCandidates}
% \SetKwFunction{checkCorrectSCG}{checkCorrectSCG}
% \SetKwFunction{sampleEdges}{sampleEdges}
% \SetKwFunction{checkMetaModel}{checkMetaModel}
% \SetKwFunction{complete}{complete}
% \SetKwFunction{prune}{prune}
% \SetKwFunction{size}{size}
% \newcommand{\pluseq}{\mathrel{+}=}


% \SetKwData{lm}{$\mathcal{L}$}
% \SetKwData{mm}{$\mathcal{TM}$}

% \SetKwData{extendedEOs}{ext}
% \SetKwData{incompleteEOs}{incomplete}
% \SetKwData{completeEOs}{complete}

% \SetKwData{extendedEO}{$\tilde\varepsilon$}
% \SetKwData{eo}{op}


% \function \generateCandidates{$\varepsilon$, \lm, \mm}:\\
% \Begin{
% \KwIn{$\varepsilon$ - given context serialization\\
% \lm - fine-tuned language model\\
% \mm - metamodel} 

% \KwOut{$[\varepsilon_1,\dots,\varepsilon_n]$ - list of candidates} 
      
%     \incompleteEOs $\gets$ [$\varepsilon$]\tcc*{set of incomplete edit operations} 
%     \completeEOs $\gets$ [] \tcc*{set of complete edit operations} 
%     \While{\size{\incompleteEOs} $>0$}{       
%         \extendedEOs $\gets$ []\tcc*{set of extended edit operations} 
%         \ForEach{\eo $\in$ \incompleteEOs}{
%          \extendedEOs $\pluseq$ \sampleEdges{\lm, \eo}\;
%          \extendedEOs $\gets$ \checkCorrectSCG{\extendedEOs}\;
%          \extendedEOs $\gets$ \checkMetaModel{\mm, \extendedEOs}\;
%          \extendedEOs $\gets$ \prune{\extendedEOs, \completeEOs}\;
%          \incompleteEOs $\gets$ []\;
%          \ForEach{\extendedEO \in \extendedEOs}{
%            \eIf{\complete{\extendedEO}}
%             {\completeEOs $\pluseq$ \extendedEO \;}
%             {\incompleteEOs $\pluseq$ \extendedEO \;}
%           }
%         }      
%     }
%     \Return{\completeEOs}
% }
% \caption{Pseudocode for the candidate generation.\label{lst:candidateGeneration}}
% \end{algorithm}
% %\vref{lst:candidateGeneration}

==> Content/approach_original.tex <==





We address the problem of automatically identifying \eo{s} from a graph mining perspective. 
As discussed in \secref{sec:background}, we will work with labeled graphs instead of typed graphs. There are some limitations related to this decision, which we discuss in \secref{sec:limitations}.

%Given such a decomposition, the actual differences are compressed in some sense. We suppose that a set of relevant \eo{s} that we want to find in the model repository should lead a high compression of the repository. A little bit sloppy this assumption can be justified by two truisms: A good \eo{} should be reused very often (and therefore be frequent) and a good \eo{} should also be not too small in terms of the meta-model in order reduce the modeling efforts. Still being sloppy, the compression is the product of these two quantities therefore justifying the assumption\footnote{There is a lot more support for this assumption, e.g., Solomonoff's theory of inductive inference.}. In this study, we will validate our believe empirically (see section \ref{sec:evaluation}). 

\textsc{Ockham} consists of the five steps illustrated with a running example in \figref{fig:approach}.
Our main technical contributions are Step 2 and Step 4. For Step~1, Step~3, and Step~5 we apply existing tooling: \textsc{SiDiff}, \textsc{Gaston}, and \textsc{Henshin} (cf.~\secref{sec:background}).

% \begin{enumerate}
%     \item Compute model differences of two successive model revisions.
%     \item Compute ``Simple Change Graphs''(SCGs) for the differences.
%     \item Apply frequent connected subgraph mining to the SCGs.
%     \item Filter and rank ``relevant'' subgraphs based on compression.
%     \item Generate edit operations out of the subgraphs of the SCG.
% \end{enumerate}

\begin{figure*}[ht]
			\centering
			\includegraphics[width=\columnwidth]{pics/Approach-Illustration.png}
			\caption{The 5-step process for mining \eo{s} with \textsc{Ockham}.}
			\label{fig:approach}
\end{figure*}

%\begin{remark}
%We will use the terms element and object for models interchangeably to describe an instance of a class. When we mean the graph representation of the object, we will speak about a node instead of object.
%\end{remark}

%%%%%%%%%%%%%%%% Step 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 1: Compute Structural Model Differences}: 
To learn a set of edit operations in an \emph{unsupervised} manner,
\textsc{Ockham} analyzes model changes that can be extracted from a model's development history. For every pair of successive model versions  $n$ and $n+1$ in a given model history, we calculate a {\em structural model difference} $\Delta(n,n+1)$ to capture these changes. As we do not assume any information (e.g., persistent change logs) to be maintained by a model repository, we use a state-based approach to calculate a structural difference, %$\Delta(n,n+1)$
which proceeds in two steps~\citep{Kehrer2015}. First, the corresponding model elements in the model graphs $G_{n}$ and $G_{n+1}$  are determined using a model matcher~\citep{kolovos2009different}. Second, the structural changes are derived from these correspondences: All the elements in $G_{n}$ that do not have a corresponding partner in $G_{n+1}$ are considered to be deleted, whereas, vice versa, all the elements in $G_{n+1}$ that do not have a corresponding partner in $G_{n}$ are considered to be newly created.

For further processing in subsequent steps, we represent a structural difference $\Delta(n,n+1)$ in a graph-based manner, referred to as {\em difference graph}~\citep{ohrndorf2021history}. A difference graph $G_{\Delta(n,n+1)}$ is constructed as a unified graph over $G_{n}$ and $G_{n+1}$. That is, corresponding elements being preserved by an evolution step from version $n$ to $n+1$ appear only once in $G_{\Delta(n,n+1)}$  (indicated by the label prefix ``Preserve\_''), while all other elements that are unique to model $G_{n}$ and $G_{n+1}$ are marked as deleted and created, respectively (indicated by the label prefixes ``Add\_'' and ``Remove\_'').

% Example
For illustration, assume that the architectural model shown in \figref{fig:difference-graph} is the revised version $n+1$ of a version $n$ by adding the ports along with the connector and its associated requirement. \figref{fig:approach} illustrates a matching of the abstract syntax graphs of the model versions $n$ and $n+1$. For the sake of brevity, only correspondences between nodes in $G_{n}$ and $G_{n+1}$ are shown in the figure, while two edges are corresponding when their source and target nodes are in a correspondence relationship. The derived difference graph $G_{\Delta(n,n+1)}$ is illustrated in \figref{fig:approach}. For example, the corresponding nodes of type {\sf Component} occur only once in $G_{\Delta(n,n+1)}$, and the nodes of type {\sf Port} are indicated as being created in version $n+1$.
%\textbf{Implementation:}
\par
Our implementation is based on the Eclipse Modeling Framework. We use the tool \textsc{SiDiff} \citep{schmidt2008constructing, kehrer2012adaptability} to compute structural model differences. \changed{Our requirements on the model differencing tool are: $(1)$ support for EMF,  $(2)$ the option to implement a custom matcher, because modeling tools such as \textsc{MagicDraw} usually provide IDs for every model element, which can be employed by a custom matcher, and $(3)$ an approach to semantically lift model differences based on a set of given \eo{s}, because we intend to use the semantic lifting approach for the compression of differences in the project mentioned in \secref{sec:case-study}. Other tools such as \textsc{EMFCompare} could also be used for the computation of model differences and there are no other criteria to favour one over the other. An overview of the different matching techniques is given by \cite{kolovos2009different}; a survey of model comparison approaches is given by \cite{Stephan2013survey}.}

%%%%%%%%%%%%%%%% Step 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 2: Derive Simple Change Graphs}:
Real-world models maintained in a model repository, such as the architectural models in our case study, can get huge. It is certainly fair to say that, compared to a model's overall size, only a small number of model elements is actually subject to change in a typical evolution step. Thus, in the difference graphs obtained in the first step, the majority of difference graph elements represent model elements that are simply preserved. To this end, before we continue with the frequent subgraph mining in Step 3, in Step 2, difference graphs are reduced to {\em simple change graphs} (SCGs) based on the principle of \emph{locality relaxation}:  only changes that are ``close'' to each other can result from the application of a single \eo{}. We discuss the implications of this principle in \secref{sec:limitations}. By ``close'', we mean that the respective difference graph elements representing a change must be directly connected (i.e., not only through a path of preserved elements). Conversely, this means that changes being represented by elements that are part of different connected components of a simple change graph are independent of each other (i.e., they are assumed to result from different edit operation applications).

More formally, given a difference graph $G_{\Delta(n,n+1)}$, a simple change graph $SCG_{\Delta(n,n+1)} \subseteq G_{\Delta(n,n+1)}$ is derived from $G_{\Delta(n,n+1)}$ in two steps. First, we select all the elements in $G_{\Delta(n,n+1)}$ representing a change (i.e., nodes and edges that are labeled as ``Remove\_*'' and ``Add\_*'', respectively). In general, this selection does not yield a graph, but just a graph fragment $F \subseteq G_{\Delta(n,n+1)}$, which may contain dangling edges. % when the source or target node of a changed edge is a preserved node not included in $F$. 
Second, these preserved nodes are also selected to be included in the simple change graph. Formally, the simple change graph is constructed as the boundary graph of $F$, which is the smallest graph $SCG_{\Delta(n,n+1)} \subseteq G_{\Delta(n,n+1)}$ completing $F$ to a graph~\citep{Kehrer2015}. 
The derivation of a simple change graph from a given difference graph is illustrated in the second step of \figref{fig:approach}. %Preserved elements that are not directly connected to changed elements are not present in the simple change graph, such as the node of type {\sf Component} and its incident edge. Moreover, preserved edges whose source and target nodes are also preserved are also not present in the simple change graph. On the contrary, all the added nodes are included in the simple change graph. Likewise, added edges are included, together with three boundary nodes of types {\sf Component} and {\sf Package} such that the simple change graph is a graph and not just a graph fragment. 
In this example, the simple change graph comprises only a single connected component. In a realistic setting, however, a simple change graph typically comprises a larger set of connected components, like the one illustrated in Step 3 of \figref{fig:approach}.

%\textbf{Implementation:} 
%We have implemented a generator for the SCGs in EMF.

% \textbf{Implementation:}  We implement a generator for the Simple Change Graphs in EMF.
% In our implementation, we loop through all the changes in the symmetric difference and for each change $c$, we add nodes and edges as below:

% \begin{itemize}
%     \item \textbf{AddNode}: For an AddNode change, we add a node with label $Add\_\{TypeName\}$ to the graph. 
%     \item \textbf{RemoveNode}: Similarly, for a RemoveNode change, we add a node with label $Remove\_\{TypeName\}$ to the graph.
%     \item \textbf{AddEdge}: For a change of type AddEdge, the source object and the target object of the added reference have to be either preserved or also been added to the model $m_{i+1}$.  If the source/target node have not yet been added to the graph, we add a node $v_{source}$/$v_{target}$ with the labels $Add\_\{TypeName\}$ or $Preserve\_\{TypeName\}$, respectively. We then add an edge $e=( v_{source}, v_{target})$ between source and target node to the edge set $E$ of the graph. 
%     \item \textbf{RemoveEdge}: Similarly, we add an edge for a change $c$ of type RemoveEdge but the source and target nodes can be either removed or preserved in this case.
%     \item \textbf{AttributeValueChange}: An attribute value needs to belong to a preserved object in the model. The corresponding $Preserve\_\{TypeName\}$ node is added to the graph if it is not yet there. Then, we will add a node with label $Change\_\{AttributeName\}\_On\_\{TypeName\}$. The pre\-served node and the node representing the changed attribute will then be connected by an edge with the same label.
% \end{itemize} 

%%%%%%%%%%%%%%%% Step 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 3: Apply Frequent Connected Subgraph Mining}:
%Using the previous two Steps for a given model repository, which for each model contains a set of model revisions, we can compute a set of SCGs. These change graphs contain information about fine-grained, meta-model based changes between two successive revisions of models.
%We believe that these fine-grained changes can be grouped to more coarse-grained changes. In the example in Figure \ref{fig:change-graph}, a connector, together with its ports and a requirement are added. The underlying idea of the approach is that changes which can be \textit{grouped together} should also frequently \textit{appear together} in our model differences.
When we apply the first two steps to a model history, we obtain a set of simple change graphs 
\begin{equation*}
    \big\lbrace SCG_{\Delta(n,n+1)} \,\mid\, n \in \lbrace 1,\dots ,N-1\rbrace\big\rbrace \, \text{,}
\end{equation*}
where N is the number of revisions in the repository. In this set, we want to identify recurring patterns and therefore find some frequent connected subgraphs. A small support threshold might lead to a huge number of frequent subgraphs. For example a support threshold of one would yield every subgraph in the set of connected components. This does not only cause large computational effort, but also makes it difficult to find relevant subgraphs. As it would be infeasible to recompute the threshold manually for every dataset, we pre-compute it by running an approximate frequent \textit{subtree miner} for different thresholds up to some fixed size of frequent subtrees. We fix the range of frequent trees and adjust the threshold accordingly. Alternatively, a relative threshold could be used, but we found in a pilot study that our pre-computation works better in terms of average precision. We discuss the effect of the support threshold further in \secref{sec:discussion}.
%This gives us a lower bound of possible frequent subgraphs (every tree is also a graph). We perform some binary search for the threshold until we find a moderate number of subtrees. We use this threshold then for the exact subgraph mining. This effectively replaces the support threshold hyper-parameter by a hyper-parameter $max\_st$ which satisfies 
% \begin{equation*}
% |ST(level=8, miner)| < max\_st,
% \end{equation*} where $ST(level=8, miner)$ denotes the number of subtrees found up to level (number of nodes) 8 with the frequent subtree miner used. We therefore don't need to (manually) find a good support threshold for the datasets and in many cases, we can be sure that the miner is able to terminate in a reasonable amount of time.
We run the frequent subgraph miner for the threshold found via the approximate tree miner. Step 3 of \figref{fig:approach} shows this for our running example. We start with a set of connected components, and the graph miner returns a set of frequent subgraphs, namely $\{g_1,g_2,g_3\}$ with $g_1 \subset g_2 \subset g_3$.
%\textbf{Implementation:} 
We use the \textsc{Gaston}~\citep{Nijssen2005} graph miner, since it performed best (in terms of runtime) among the miners that we experimented with (\textsc{gSpan}, \textsc{Gaston}, and \textsc{DIMSpan}) in a pilot study. \changed{In our pilot study, we ran the miners on a small selection of our datasets and experimented with the parameters of the miners. For many datasets, \textsc{gSpan} and \textsc{DIMSpan} did not terminate at all (we canceled the execution after 48h). \textsc{Gaston} (with embedding lists) was able to terminate in less then 10s on most of our datasets but consumes a lot of memory, typically between 10GB--25GB, which was not a problem for our 32GB machine in the pilot study. To rule out any effects due to approximate mining, we considered only exact miners. Therefore, we also could not use \textsc{Subdue} \citep{Ketkar2005}, which directly tries to optimize compression. Furthermore, \textsc{Subdue} was not able to discover both \eo{s} in the second experiment (see \secref{sec:evaluation}), without iterative mining and allowing for overlaps. Enabling these two options, \textsc{Subdue} did not terminate on more than 75\% of the pilot study datasets}. 
For frequent subtree mining, we use \textsc{Hops} \citep{Welke2020} because it provides low error rates and good runtime guarantees.\par
%%%%%%%%%%%%%%%% Step 4 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 4: Select the most Relevant Subgraphs}:
Motivated by the \emph{minimum description length principle}, \changed{which has been successfully applied to many different kinds of data}~\citep{grunwald2007minimum}, the most relevant patterns should not be the most frequent ones but the ones that give us a maximum compression for our original data \citep{Djoko1994}. 
That is, we want to express the given SCGs by a set of subgraphs such that the description length for the subgraphs together with the length of the description of the SCGs in terms of the subgraphs becomes minimal. \changed{This reasoning can be illustrated by looking at the corner cases: $(1)$ A single change has a large frequency but is typically not interesting. $(2)$ The entire model difference is large in terms of changes but has a frequency of only one and is typically also not an interesting \eo{}. ``Typical \eo{s}'' are therefore somewhere in the middle. We will use our experiments in \secref{sec:evaluation} to validate whether this assumption holds.
% More formally:
% \begin{definition}
% Given a SCG $G=(V_G,E_G)$ and a set $SG := \lbrace g_1, \dots, g_k \rbrace$ of subgraphs, we define the subgraph decomposition $G/SG$ of $G$ to be a graph $(V_{G/SG}, E_{G/SG})$, where the nodes in $V_{G/SG}$ are instances of elements of $SG$, i.e., the subgraphs, in $G$,
% and for each two subgraphs that are connected in $G$, we have an edge $e$ in  $E_{G/SG}$. For a graph $g$ we denote the set of nodes by $V_g$ and the set of edges by $E_g$.
% \end{definition}
% \begin{definition}
% We define the description length of a subgraph decomposition $G/SG$ by
% \begin{equation}
%     L(G/SG) = L(SG) + L(G|SG),
% \end{equation} where $L(SG)$ and $L(G|SG)$ are defined as follows:
% $$L(SG) = \sum_{g \in SG}  (|V_g| + |E_g|)$$
% $$L(G|SG) = |V_{G/SG}| + |E_{G/SG}|$$
% \end{definition}
% The maximum compression criterion then means to find $SG$ such that $L(G|SG)$ is minimal.
% % \begin{equation}
% % \label{eq:optimization}
% % \underset{SG}{\operatorname{arg min}}\ L(G/SG)
% % \end{equation}
% \begin{remark}
% In the definitions above, we don't take the description length of the labels into account and assume equal description length for each label.
% \end{remark}
%There are two problems with this approach. The first one is, that the original SCG can not be completely reconstructed out of the reduced graph, since some additional information is needed on how two subgraphs are connected together in the original graph. 
%The second problem is that there are too many possible combinations over which the minimum has to be found.
%One problem with the decomposition of the whole difference graph in terms of subgraphs is that there are too many possible combinations over which the minimum has to be found.
We define the compression value by}
\begin{equation*}
    \operatorname{compr}(g) = \big({\operatorname{supp}}(g)-1\big) \cdot \big(\mid V_g \mid +  \mid E_g \mid\big) \, \text{,}
\end{equation*}
where ${\operatorname{supp}}(g)$ is the support of $g$ in our set of input graphs (i.e., the number of components in which the subgraph is contained). The ``$-1$'' in the definition of the compression value comes from the intuition that we need to store the definition of the subgraph, to decompress the data again. \changed{The goal of this step is to detect the subgraphs from the previous step with a high compression value.}
%That is, we assume that the subgraphs in a set $SG$ which fulfills the compression criterion %equation \ref{eq:optimization} 
%provide a high compression. 
%Of course, this is not necessarily true. For example, if we have a subgraph $g_k$ with a very high compression and we reduce our set of connected components by this subgraph, we might be left with many ``tiny'' nodes, that can not be further compressed. So this subgraph decomposition might in the end have a larger description length as some other subgraph decomposition $\lbrace \tilde{g_1}, \dots, \tilde{g_m} \rbrace$ but where each of the subgraphs $\tilde{g_i}$ has a lower compression $cr(\tilde{g_i}) < cr(g_k) \forall j \in 1, \dots, m$. 
%Here again, we take the standpoint from the beginning of the section that a good \eo{} should not be not too small and should often be reused. To reduce the risk of missing some relevant \eo{}, we also look at edit operations that are only frequent but not necessarily among the ones with the best compression. The remaining \eo{s} that we will miss are then the ones that are large but not frequent and the ones that small and not frequent. For the first class, i.e., the infrequent large induced subgraphs, it is likely that these are comprised of smaller, more frequent subgraphs (i.e., we have some hierarchy's of \eo{s}). The second class is not relevant for our use case, since they do not help us to make the model difference easier to understand. %Furthermore, after identifying a set of \eo{s} in the next Step, the approach by Kehrer et al. (\cite{Kehrer2011}) can be used to decompose the model difference. If there is some ``remainder'' of changes that are not part of some \eo{}, these remainders can be manually investigated.
%We then also experiment with some further pruning heuristics, to reduce the number of results.
%\textit{Cohesion assumption:} When an induced subgraph has some nodes that have a much smaller degree\footnote{the degree of a node of an undirected graph is the number of adjacent nodes} within the induced subgraph than their embedding in the original graph, it is likely that these nodes are part of another \eo{}. By much smaller, we mean that  $d(v) < 2 \cdot d(\tilde{v}) + \epsilon$ for some $\epsilon \in \mathbb{N}$, where $\tilde{v}$ is the embedding of $v$ in the SCG.\\
%We then do not count this instance for the support of the corresponding tree. Note, that this kind of \textit{cohesion assumption} is not always true. For example, in our models we might add some ``container-like'' objects. The \eo{} of adding this container-like objects will then be pruned (more precisely their corresponding subgraphs in the SCG) when some objects are added to the container in the same model revision. That means, the \eo{} of adding the container might be pruned completely in the end. Therefore, the effect of this pruning needs to be investigated empirically on our datasets.
Subgraphs are organized in a \emph{subgraph lattice}, where each graph has pointers to its direct subgraphs. Most of the subgraph miners already compute a subgraph lattice, so we do not need a subgraph isomorphism test here. Due to the downward closure property of the support, all subgraphs of a given (sub-)graph have, at least, the same frequency (in transaction-based graph mining). When sorting the output, we need to take this into account, since we are only interested in the largest possible subgraphs for some frequency. \inExtension{These largest possible subgraphs for some frequency are called closed subgraphs and typically the number of closed subgraphs is much smaller than the number of all frequent subgraphs \citep{Yan2003}.}{}{} Therefore, we prune the subgraph lattice. % as in Listing \ref{lst:pruning}.
The resulting list of recommendations is then sorted according to the compression value. \changed{Other outputs are conceivable, but in terms of evaluation, a sorted list is a typical choice for a recommender system~\citep{schroder2011setting}.}  \par
More technically, let $SG$ be the set of subgraphs obtained from Step~3, we then remove all the graphs in the set 
\begin{align*}
%\begin{split}
SG^- = \big\lbrace g &\in SG \,\mid\, \exists \tilde g \in SG \text{, with } g \subseteq \tilde g \\
&\wedge \operatorname{supp}(g) = \operatorname{supp}(\tilde g) 
 \wedge \operatorname{compr}(g) \leq \operatorname{compr}(\tilde g) \big \rbrace\text{.}
%\end{split}
\end{align*}

Our list of recommendations is then $SG \setminus SG^-$, sorted according to the compression metric.

% \noindent\begin{minipage}{.48\textwidth}
% \begin{lstlisting}[caption=Lattice pruning,label={lst:pruning},frame=tlrb, basicstyle=\sf, breaklines=true, language=Python, columns=fullflexible]{lst:pruning}
% # dict with keys = subgraphs and values = (compr, freq, children)
% lattice = {k: v for k, v in sorted(lattice.items(), key=compr, reverse=True)}
% for subgraph in list(lattice.keys()):
%   if subgraph in lattice.keys():
%       df_pruning(lattice, subgraph)

% # prune in a depth-first manner
% def df_pruning(lattice, subgraph):
%     for child in (set(lattice[subgraph][2]) & set(lattice.keys())):
%         df_pruning(lattice, child)
%         if lattice[child][1] <= lattice[subgraph][1]:
%             lattice.pop(child)
% \end{lstlisting}
% \end{minipage}\hfill

% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=\columnwidth]{pics/pruned_lattice.png}
% 			\caption{We prune less or equal frequent subgraphs in the subgraph lattice.}
% 			\label{fig:pruned-lattice}
% 			\vspace{-1em}
% \end{figure}

For our running example in Step 4 of \figref{fig:approach}, assume that the largest subgraph $g_3$ occurs 15 times (without overlaps). Even though the smaller subgraph $g_1$ occurs twice as often, we find that $g_3$ provides the best compression value and is therefore ranked first. Subgraph $g_2$ will be pruned, since it has the same support as its supergraph $g_3$, but a lower compression value.
%\textbf{Implementation:}
We implement the compression computation and pruning using the \emph{NetworkX}\footnote{\url{https://networkx.org/}} Python library.

% TODO this needs to be explained better and edge also have to be taken into account
%Last but not least, many (false) subgraphs might have a large overlap with the right subgraphs. We therefore favor subgraphs that have a large distance to the subgraphs listed already.
%To this end, we define the node label distance of two graphs $g_1$ and $g_2$ by 
%\begin{equation}
%    d(g_1, g_2) = \lambda(V_{g_1})\ \Delta\  \lambda(V_{g_2}),
%\end{equation}
%where $\lambda(V_t)$ are all the node labels of a graph $t$ and $\Delta$ is the symmetric difference. More precisely, when a label appears $n$ times in $g_1$ and $m$ times in $g_2$, we add %$\operatorname{max}(n-m, m-n)$ to the node label distance $d$.

%%%%%%%%%%%%%%%% Step 5 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Step 5: Generate Edit Operations}:
As a result of Step 4, we have an ordered list of ``relevant'' subgraphs of the simple change graphs. We need to transform these subgraphs into model transformations that specify our learned \eo{s}. As illustrated in Step~5 of \figref{fig:approach}, the subgraphs can be transformed to Henshin transformation rules in a straightforward manner. \inExtension{At this point, we can also use the information from the meta-model to complete the \eo{s}. For example, when a created element requires another element or attribute, which is not yet present, it can be added. This is done similarly to the derivation of consistency preserving \eo{s} by \cite{Kehrer2016}.}{}{} \changed{We use \textsc{Henshin} because it is used for the semantic lifting approach in our case study from Sec. \ref{sec:case-study}. In principle, any transformation language that allows us to express endogenous, in-place model transformations could be used. A survey of model transformation tools is given by \cite{kahani2019survey}.}

% \begin{remark}
% For this study, we consider subgraphs of Simple Change Graphs to be equivalent to the \eo{s}, i.e., we ignore things like inheritance which have a meaning for \eo{s} but not yet for the SCGs. We therefore sometimes use the concepts of the subgraphs and \eo{s} interchangeably.
% \end{remark}

%\textbf{Implementation:} 
%We compute \textsc{Henshin} graph transformations out of graphs from the previous Step. 

%\begin{figure}[ht]
%			\centering
%			\includegraphics[width=\columnwidth]{pics/RemoveInterface.png}
%			\caption{\textsc{Henshin}-rule to remove a port (interface) from a component.}
%			\label{fig:\textsc{Henshin}-removeport}
%\end{figure}


==> Content/approximate_mining.tex <==
%\subsubsection{Experiment 3 (WIP) - TODO Include experiment regarding approx. mining in this paper or extra paper? }
%Frequent connected subgraph mining is a highly computationally intensive tasks. Especially, if we want to find larger groups of changes, the task quickly becomes computationally infeasible.
%We therefore also compare approximate frequent subgraph mining to the exact frequent subgraph mining in step 3 of our approach. 
%We use the algorithms by Welke et al. (\cite{Welke2019})  and \cite{Welke2020})\footnote{There are also graph miners (\cite{Ketkar2005}) that are directly based on a compression metric. Unfortunately, for our datasets, Subdue performed worse in a pilot study}. 
%These algorithms are frequent subtree miners with the property that a tree, identified as frequent by the algorithm, is also a frequent tree but not necessarily all frequent trees are discovered. 
%In our case, we are interested frequent \textit{induced} subgraphs, i.e., all edges between the nodes that are present in the original graph are also present in the subgraph.
%Furthermore, we will usually find many frequent trees, which are contained in a larger frequent tree\footnote{Actually this so called downward closure property holds in general for these algorithms.}. 
%Also, we are usually interested in the largest graph with a certain frequency and not all of its subgraphs with the same frequency.
%For all of these reasons, we need to perform some post-processing on our frequent trees discovered by the tree miners.
%We use some embedding operator (i.e., an operator which gives us an occurrence of the subtree in a given graph, if any), to find occurrences of the trees in the set of connected components. For this study, we also used the embedding operator from Welke et al. \cite{Welke2020}. For every embedding that we find, we can easily compute the induced subgraph. We then recount the induced subgraphs, since even for a frequent tree, the subgraphs might not be frequent because we might have many different kind of induced subgraphs corresponding to a frequent subtree\footnote{Luckily, every spanning tree of a frequent connected induced subgraph must also be frequent.}. 

%\begin{remark}
%We only need to recompute the embeddings, since we are using the tree miner as a black box for this study. Therefore, this additional computationally complex step is just an implementation detail but not a shortcoming of the approach. We could also modify the tree miner to return the induced subgraphs instead of the frequent trees, which we will leave for future work.
%\end{remark}

==> Content/background_original.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}\label{sec:background}
In this section, we provide basic definitions that are important to understand our approach presented in \secref{sec:appraoch}.

\subsection{Model Evolution}
We are interested in \eo{s} as an important subclass of model transformations. An \emph{edit operation} is an in-place %(i.e., within one model) 
model transformation and usually represents regular evolution \cite{visser2007model} of models. For example, when moving a method from one class to another in a class diagram, also a sequence diagram that uses the method in message calls between object lifelines needs to be adjusted accordingly. To perform this in a single edit step, one can create an \eo{} that executes the entire change, including all class and sequence diagram changes.
Some tasks can even be completely automatized and reduced to the definition of \eo{s}: Edit operations are used for model repair, quick-fix generation, auto completion~\cite{ohrndorf2021history, hegedus2011quick, Kogel2016}, model editors \cite{taentzer2007generating, ehrig2005generation},  operation-based merging \cite{koegel2009operation, schmidt2009history}, model refactoring \cite{Mokaddem2018, Arendt2013},  model optimization \cite{burdusel2018mdeoptimiser}, meta-model evolution and model co-evolution \cite{rose2014graph, arendt2010henshin, herrmannsdoerfer2010extensive, getir2018supporting, kolovos2010taming}, semantic lifting of model differences \cite{Kehrer2011, kehrer2012understanding, ben2012search, langer2013posteriori, khelladi2016detecting}, model generation \cite{pietsch2011generating}, and many more.

A major class of \eo{s} are model refactorings, which induce syntactical changes without changing a models' semantics. Other classes of \eo{}s include recurring bug fixes and evolutionary changes. %(i.e., adding new functionality). 

In a classification by \cite{visser2007model}, \eo{s} can describe regular evolution, that is, ``the modeling language is used to make changes'', but they are not meant to describe meta-model evolution, platform evolution, or abstraction evolution. More technically, in Mens et al.'s taxonomy~\citep{Mens2006}, \eo{s} can be classified as endogenous (i.e., source and target meta-model are equal), in-place (i.e., source and target model are equal) model transformations. 
%They can be mathematically formalized by graph transformations on typed graphs. Due to space constraints, we refer the readers to the work of Bierman et al. \cite{Biermann2012} and Ehrig et al. \cite{Ehrig2004} for details.
For the purpose of this paper, we define an \eo{} as an in-place model transformation which represents regular model evolution.

The model transformation tool \textsc{Henshin}~\citep{arendt2010henshin} supports the specification of in-place model transformations in a declarative manner. It is based on graph transformation concepts~\citep{Ehrig2004}, and it provides a visual language for the definition of transformation rules, which is used, for example, in the last step of \figref{fig:approach}. Roughly speaking, transformation rules specify graph patterns that are to be found and created or deleted.


\subsection{Graph theory}
As usual in MDE, we assume that a meta-model specifies the abstract syntax and static semantics of a modeling language. Conceptually, we consider 
%an instance of a meta-model (i.e., a model) 
a model as a typed graph (aka. abstract syntax graph), in which the types of nodes and edges are drawn from the meta-model. \figref{fig:difference-graph} illustrates how a simplified excerpt from an architectural model of our case study from \secref{sec:case-study} in concrete syntax is represented in abstract syntax, typed over the given meta-model. 

\begin{figure}[ht]
			\centering
			\includegraphics[width=\columnwidth, clip]{pics/concrete_vs_abstract.png}
			\caption{We consider models as labeled graphs, where labels represent types of nodes and edges defined by a meta model. For the sake of brevity, types of edges are omitted in the figure.}
			\label{fig:difference-graph}
\end{figure}

We further assume models to be correctly typed. %, in our notion of a graph used throughout the paper,
We abstain from a formal definition of typing using type graphs and type morphisms \citep{Biermann2012}, though. Instead, to keep our basic definitions as simple as possible, we work with a variant of labeled graphs in which a fixed label alphabet represents node and edge type definitions of a meta-model.
%\begin{definition}
Given a label alphabet $L$, a \textit{labeled directed graph} $G$ is a tuple $(V,E,\lambda)$, where $V$ is a finite set of nodes, $E$ is a subset of $V \times V$, called the edge set, and $\lambda: V \cup E \to L$ is the labeling function, which assigns a label to nodes and edges. 
%In this study, we will mainly work with \textit{undirected} graphs. In this case, the edge set $E$ is consisting of a set of vertices, i.e., $\lbrace u,v\rbrace$ is the undirected edge connecting $u$ and $v$. 
%\end{definition}
If we are only interested in the structure of a graph and typing is irrelevant, we will omit the labeling and only refer to the graph as $G = (V,E)$.

%We furthermore need the definition of a subgraph and a subgraph isomorphism:

%\begin{definition}
Given two graphs $G = (V,E,\lambda)$ and $G' = (V',E',\lambda')$, $G'$ is called a \emph{subgraph} of $G$, written $G' \subseteq G$, if $V' \subseteq V$, $E' \subseteq E$, and 
$\lambda(x) = \lambda'(x)$ for each $x \in V' \cup E'$.
%labelled over the same alphabet. 
%\label{def:subgraph}
%\end{definition}
% Two graphs $G_1$ and $G_2$ are said to be \textit{isomorphic}, if there is a bijection 
% $\phi: V_{G_1} \to V_{G_2}$ with 
% \begin{equation}\label{eq:sg_isomorph}
%     (\phi(u), \phi(v)) \in E_{G_2} \Leftrightarrow (u, v) \in E_{G_1}. %\forall u,v \in V_{G_1}: 
% \end{equation}
% A graph $G_2$ is said to be \textit{subgraph isomorphic} to $G_1$, $G_2 \preccurlyeq G_1$, if $G_1$ has a subgraph that is isomorphic to $G_2$. The subgraph isomorphism $\phi$ is called \textit{induced}, if furthermore equation \ref{eq:sg_isomorph} holds.
%\begin{definition}
\changed{
A \textit{(weakly) connected component} (component, for short) $C=(V_C, E_C) \subseteq G$ is an induced subgraph of $G$ in which every two vertices are connected by a \textit{path}, that is,  
%\begin{equation*}
${\forall u,v \in V_C} : {\exists n\in\mathbb{N}} \text{ s. t. } {\big\lbrace (v, v_1), (v_1, v_2), \dots ,(v_n, u)\big\rbrace} \subseteq E_C \ \cup \tilde E_C$, where $\tilde E_C$ is the set of all reversed edges, that is, $(u, v) \in E_C$ becomes $(v, u) \in \tilde E_C$.
}
%\end{equation*}
%\end{definition}
\subsection{Frequent Subgraph Mining}
We will use frequent subgraph mining as the main ingredient for \textsc{Ockham}. We distinguish between \textit{graph-transaction-based frequent subgraph mining} and \textit{single-graph-based frequent subgraph mining}.
%Graph-transaction-based frequent subgraph mining uses a collection (aka. \emph{database}) of graphs, while single-graph-based frequent subgraph mining looks for subgraphs of a single graph. 
In particular, we are considering graph-transaction-based frequent subgraph mining, which typically takes a database\inExtension{~(i.e., a set)}{}{} of graphs and a threshold $t$ as input. It then outputs all the subgraphs with, at least, $t$ occurrences in the database. 
%The target of subgraph mining is to identify subgraphs in the input with a \textit{support}, i.e., the occurrence count, higher than some \textit{support threshold}. In transaction based FSM one usually counts a subgraph only once per transaction (= graph in the collection of graphs). In our study, we will only consider transaction based FSM. Most subgraph miners work by enumerating subgraph candidates and then using some embedding operator to count the occurrences of the frequent subgraph candidate. In transaction based FSM the so called \textit{downward closure property} can be employed when enumerating the subgraphs. This property states that for a frequent subgraph all of its subgraphs are frequent as well, which is a simple consequence of the definition of the support for transaction based FSM. Using this property, enumerating the subgraphs can be done by growing the subgraphs edge- or vertex-wise. When a subgraph is not frequent anymore, this subgraph does not need to be extended further. Furthermore, most of the algorithms use some pruning to avoid enumerating subgraph candidates redundantly (see for example gSpan \cite{Yan2002}).
An overview of frequent subgraph mining algorithms can be found in the literature \citep{Jiang2008}. \changed{
A general introduction to graph mining is given by \cite{cook2006mining}, who also proposed a compression-based subgraph miner called \textsc{Subdue}~\citep{Ketkar2005}.  \textsc{Subdue} has also been one of our main inspirations for a compression-based approach. %We will detail in \secref{sec:appraoch} why we did not use the Subdue tool for our approach.
}\textsc{Ockham} is based on \textsc{Gaston} \citep{Nijssen2005}, which mines frequent subgraphs by first focusing on frequent paths, then extending to frequent trees, and finally extending the trees to cyclic graphs.
\inExtension{Since deciding if a graph $G'$ is a subgraph of another graph $G$ is already $\mathcal{NP}$-complete, there is no polynomial time algorithm for frequent subgraph mining. Usually, if there are large graphs in the database or the threshold is too low, the problem becomes computationally intractable. In these situations, the number of subgraphs typically also becomes intractable. In many scenarios though, one is not interested in a complete list of all frequent subgraphs. In these cases, huge graphs in the database can be filtered out or the threshold can be increased such that the frequent subgraph mining becomes feasible.}{}{}

\subsection{Model Transformations and Edit Operations}\label{sec:editoperations}
%In this subsection, the term \textit{model} refers to an Eclipse Modeling Framework (EMF) model. 
The goal of \textsc{Ockham} is to learn domain-specific \textit{\eo{s}} from model histories. In general, \eo{s} can be informally understood as editing commands that can be applied to modify a given model. In turn, a difference between two model versions can be described as a (partially) ordered set of applications of \eo{s}, transforming one model version into the other. Comparing two models can thus be understood as determining the applications of the \eo{} applications that transform one model into the other.
%An \eo{} is \textit{consistency preserving}, if it transforms a consistent model (i.e., conforming to the meta-model) to another consistent model.
A major class of \eo{s} are model refactorings, which induce syntactical changes without changing a models' semantics. Other classes of \eo{}s include recurring bug fixes and evolutionary changes. %(i.e., adding new functionality). 

In a classification by \cite{visser2007model}, \eo{s} can describe regular evolution, that is, ``the modeling language is used to make changes'', but they are not meant to describe meta-model evolution, platform evolution, or abstraction evolution. More technically, in Mens et al.'s taxonomy~\citep{Mens2006}, \eo{s} can be classified as endogenous (i.e., source and target meta-model are equal), in-place (i.e., source and target model are equal) model transformations. 
%They can be mathematically formalized by graph transformations on typed graphs. Due to space constraints, we refer the readers to the work of Bierman et al. \cite{Biermann2012} and Ehrig et al. \cite{Ehrig2004} for details.
For the purpose of this paper, we define an \eo{} as an in-place model transformation which represents regular model evolution.

The model transformation tool \textsc{Henshin}~\citep{arendt2010henshin} supports the specification of in-place model transformations in a declarative manner. It is based on graph transformation concepts~\citep{Ehrig2004}, and it provides a visual language for the definition of transformation rules, which is used, for example, in the last step of \figref{fig:approach}. Roughly speaking, transformation rules specify graph patterns that are to be found and created or deleted.
%To formalize the concept of edit operations, we first have to formalize the concept of a model. Usually a model can be represented in a \textit{concrete (visual) syntax} and an \textit{abstract syntax}. The concrete syntax defines how the model is presented to a user. The abstract syntax describes the model in terms of its meta-model. The meta-model can be seen as a \textit{type graph} for the model. In the abstract syntax, the model is then a \textit{typed graph}. A class in the meta-model corresponds to a type of a node in this typed graph. Similarly, the type of an edge in the typed graph corresponds to the association relationship in meta-model (type graph). The mathematical rigorous formalization as well as an informal introduction of these concepts is given in the work of Biermann et al. \cite{Biermann2012} and, also taking attributes into account, in Ehrig et al. \cite{Ehrig2004}. 

%\begin{remark}
%In this work, we will work with simplified (and not as feature-rich) graph concepts but the work will be extended to the language of attributed typed graphs in the future.
%\end{remark}

%Using this graph-based formalization of a model an edit operation can be described as an \textit{endogenous model transformations} which can be formalized by graph transformations \cite{Biermann2012}. An endogenous model transformation transforms a model of one meta-model to another model of the same meta-model. %while for an \textit{exogenous model transformation} the meta-model for the source and target model can be different. 
%There is a rich theory behind these graph transformations and the results of this theory form the basis for tool called \textsc{Henshin}. Model transformations are described in form of so called \textit{\textsc{Henshin} rules}. An example is given in the upper part of Figure \ref{fig:change-graph}. These rules consist of a left-hand side (LHS) which describes a pattern to be matched in a graph and a right-hand side (RHS) which substitutes the LHS.
%urthermore, there can be so called \textit{positive- or negative application conditions} that extend the LHS of the rule. Informally, the application of a \textsc{Henshin} rules works as follows:

% \begin{enumerate}
%     \item The LHS of the rule (plus possibly positive- or negative application conditions) is matched in the model. There can be many matches (or none). For a concrete edit operation usually one constrains the LHS with parameters (e.g., object ids) to select a concrete match.
%     \item Nodes and edges in $LHS \backslash RHS$ are removed from the matched part of the model. By ``$\backslash$'', we mean the set minus operation on $V \cup E$.
%     \item Nodes and edges in $RHS \backslash LHS$ are ``glued'' along the preserved elements in $LHS \cap RHS$.
% \end{enumerate}

% The mathematical formalization of the graph transformation can be done by the use of the so called double-pushout construction from category theory \cite{Biermann2012}.



%One thing to note here is that the matching is done by \textsc{Henshin} using a constraint programming approach which is NP-complete. Thanks to the type information the search space for match candidates is usually small in practical examples and therefore the graph transformation approach becomes computationally feasible.

%Note that there are plenty of other approaches to model transformations, e.g., Fujaba \cite{Klein1999} or VIATRA \cite{Bergmann2015}. Furthermore, there are many approaches in the area of exogenous model transformations.

%More details about this formalization of \eo{s} can also be found in the work of Kehrer \cite{Kehrer2015}. 
%This work furthermore describes how model difference can be \textit{semantically lifted} by describing the model difference in terms of \eo{s} instead of fine-grained meta-model based differences.

%We will use model transformation to describe the evolution of models but they play a fundamental role for MDE \cite{Mens2006}. MDE makes models the central objects of the (software) development lifecycle and model transformations become a means to evolve models. Many software engineering tasks are reduced to the definition of corresponding model transformations. Just to name a few, 

% documentation (better topic?)
%data schemata and SQL scripts can be generated out of Ecore models or UML class diagrams \cite{vara2009supporting}, 

% model migration
%models for different purposes can be consistently migrated \cite{rose2014graph},

%model repair%
%inconsistencies in related artifacts can be automatically detected and repaired  \cite{ohrndorf2021history},

%V&V
%UML models can be transformed to models for which formal 
%verification and validation is possible \cite{Csertan2002},

% code generation and reverse engineering
%even behavioural source code can be generated out of models and tools like Fujaba \cite{Klein1999} also envision reverse engineering of source code.\par

% and of course many more, slicing meta-model co evolution (also migration topic), all knowledge and documentation related things, traceing,...co-change analysis, impact analysis (ohrndorf covers several of these things with his approach)




==> Content/casestudy_original.tex <==
\section{\changed{Motivation: An Industrial Scenario}}\label{sec:case-study}
Our initial motivation to automatically mine \eo{s} from model repositories arose from a long-term collaboration with practitioners from a large-scale industrial model-driven \spl{} in the railway domain. The modeling is done in \textsc{MagicDraw}\footnote{\url{https://docs.nomagic.com/}} using SysML, and there is an export to the Eclipse Modeling Framework (EMF), which focuses on the SysML parts required for subsequent MDE activities (e.g., code generation). Modeling tools such as \textsc{MagicDraw} %or Papyrus 
come with support for model versioning. In our setting, the models are versioned in the MagicDraw Teamwork Server. We therefore have access to a large number of models and change scenarios. \par 
Discussing major challenges with the engineers of the product line, we observed that some model changes appear very often together in this repository. For example, when the architect creates an interface between two components, s/he will usually add some {\sf Ports} to {\sf Components} and connect them via the {\sf ConnectorEnds} of a {\sf Connector}. Expressed in terms of the meta-model, there are 17 changes to add such an interface\inExtension{~(see \figref{fig:semantic-lifting}).}{.}{} We are therefore interested to automatically detect these patterns in the model repository. More generally, our approach, \textsc{Ockham}, is based on the assumption that it should be possible to derive ``meaningful'' patterns from the repositories.
These patterns could then be used for many applications~\changed{\cite{ohrndorf2021history, Kogel2016, taentzer2007generating, Arendt2013,  getir2018supporting, kehrer2012understanding, ben2012search, langer2013posteriori, khelladi2016detecting}}. %\cite{ohrndorf2021history, Kogel2016, taentzer2007generating, ehrig2005generation, koegel2009operation, Arendt2013,  getir2018supporting, kolovos2010taming, Kehrer2011, kehrer2012understanding, ben2012search, langer2013posteriori, khelladi2016detecting, pietsch2011generating}. 
\par
\inExtension{ 
 \begin{figure}[ht]
 			\centering
 			\includegraphics[width=\columnwidth]{pics/Semantic-Lifting.png}
 			\caption{Semantic lifting can be used to group many fine-grained changes into change sets.}
 			\label{fig:semantic-lifting}
 \vspace{-1em}
 \end{figure}
}{}{}
The background is that, in our case study, the models have become huge over time (approx. 1.2 million elements split into 100 submodels) and model differences between different products have become huge (up to 190,000 changes in a single submodel). The analysis of these differences, for example, for quality assurance of the models or domain analysis, has become very tedious and time-consuming. To speed-up the analysis of the model differences, it would be desirable to reduce the ``perceived'' size of the model difference by grouping fine-grained differences to higher-level, more coarse-grained and more meaningful changes. For this \emph{semantic lifting} of model differences, the approach by \cite{Kehrer2011}, which uses a set of \eo{s} as configuration input, can be used but the approach requires the \eo{s} to be defined already. \inExtension{Based on a set of \eo{s} this semantic lifting approach will group changes into so called \emph{change sets}.\par}{}{} 
Large model differences occurring in some of the activities in this setting have actually been our main motivation to investigate how we can derive the required \eo{s} (semi-)automatically. \par
We will use the data from this \changed{real-world project} to evaluate \textsc{Ockham} in \secref{sec:evaluation}.
% \section{Real-World Railway Case Study}\label{sec:case-study}
% Our motivation to automatically mine \eo{s} in model repositories comes from an large-scale industrial model-driven \spl{} in the railway domain. The modeling is done in MagicDraw\footnote{https://www.nomagic.com/} using the SysML modeling language but there is also an export to an Eclipse Modeling Framework based model, which only focuses on the SysML parts which are necessary for some other MDE activities, e.g., source code generation.\par 
% Many industrial \spl{s} have been organically grown, and some form of managed cloning (\cao{} with some kind of clone management in place) is used \cite{Dubinsky2013}.
% In our case study, there are only a few products, the so called train-set types and therefore a form of managed cloning using different branches of the repository for each train-set type as well as one branch for the platform model is used. The platform model is evolved by following an extractive \spl{} adoption path \cite{Apel2013}, i.e., common features are (manually) identified and regularly merged into the platform. 

% In interviews conducted with five architects and engineers of this project, four of the five participants mentioned the ``drift'' of the architecture as a major challenge (see Figure \ref{fig:model-drift}). The model drift appears as huge model differences (e.g., 180 000 changes for one single sub-model of approx. 100 sub-models in the whole project) between two train-set types or between the platform model and one of the train-set types. It can then become difficult to identify commonalities that can be lifted into the common platform (domain engineering). Also, analyzing a difference of a product and a platform, e.g., for quality assurance purposes or to merge some parts from the product into the platform or vice versa, becomes a challenging task. This can even lead to a risk of loosing the benefits of reuse if efforts related to cloning and merging exceed the savings of reuse.


% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=0.8\columnwidth]{pics/Model_Drift.png}
% 			\caption{Products and platform inevitably drift apart when using \cao{}.}
% 			\label{fig:model-drift}
% \vspace{-1em}
% \end{figure}

% We want to approach the problem of the large model differences and the drift between different products in the \spl{} by reducing the ``perceived'' size of the model difference by grouping fine-grained differences to higher-level (semantic) changes. These changes can also be classified (e.g., a change can be a violation) to support the architect or developer during the analysis and quality assurance related tasks. Furthermore, the higher-level changes can also speed-up tasks like identification of common functionalities. 
% For this semantic-lifting the approach by Kehrer et al. \cite{Kehrer2011} can be used. This reduces the problem to the definition of ``meaningful'' \eo{s}. The semantic-lifting then decomposes the model difference in terms of given \eo{s}. The most straight-forward approach to define ``meaningful'' is, to consider edit operations or edit scenarios that are performed in the modeling tools. E.g., when the architect creates an interface between two components, s/he will usually add some \emph{Ports} to \emph{Components} and connect them via the \emph{ConnectorEnds} of a \emph{Connector}. Instead of presenting the fine-grained changes (17 changes in the concrete meta-model) it is desirable to show the entire change in the model difference. We are therefore interested if our approach is able to find typical edit scenarios in this real-world setting.

==> Content/conclusion_original.tex <==

\section{Conclusion and Outlook}
We have proposed an approach, \textsc{Ockham}, for automatically deriving \eo{s} specified as in-place model transformations from model repositories. \textsc{Ockahm} is based on the idea that a meaningful \eo{} will be one that provides a good compression for the model differences. In particular, it uses frequent subgraph mining on labeled graph representation of model differences to discover frequent patterns in the model differences. The patterns are then filtered and ranked based on a compression metric to obtain a list of recommendations for meaningful \eo{s}. To the best of our knowledge, \textsc{Ockham} is the first approach for learning domain-specific edit operations in a fully \emph{unsupervised} manner, that is, without relying on any manual intervention or input from a developer or domain expert. \par
We have successfully evaluated \textsc{Ockham} in two controlled experiments using synthetic ground-truth EMF models and on a large-scale real-world case study in the railway domain. We found that \textsc{Ockham} is able to extract \eo{s} that have actually been applied before and that it discovers meaningful \eo{s} in a real-world setting. Including too large components in the difference graphs can adversely affect \textsc{Ockham} in discovering the applied \eo{s}. Performance mostly depends on the number of applied \eo{s} in a model difference. \inExtension{Furthermore, we have shown how the \eo{s} discovered by \textsc{Ockham} can be used in practical applications. For example, they can be used in a semantic lifting, to express model differences in terms of \eo{s} and therefore ``compress'' the model differences. Depending on the concrete task related to the model differences, the lifted model differences can then also be filtered for the \eo{s} of interest. The frequency distributions of \eo{s} in model differences can also be used for a high-level analysis of the model differences, for example, to discover hot spots, where a lot of functional evolution has happened.}{}{}
\textsc{Ockham} can be applied to models of any Domain-Specific Modeling Language for which model histories are available. New effective \eo{s} that are performed by the users can be learned at runtime and recommendations can be made.\par
%The tool would therefore become a self-aware system \cite{Kephart2017} which continuously adapts itself to the user needs. This self-aware tool vision forms the basis for our future research in mining \eo{}.
%Future work
For our future research, we plan to extend \textsc{Ockham} by a meta-heuristic search to identify the optimal \emph{set} of operations. \inExtension{Extending state-of-the-art frequent subgraph miners to handle concepts like inheritance, multi-object structures, and other concepts from model-driven software development will very likely improve the results of \textsc{Ockham}. Since exact frequent subgraph mining is not tractable when large connected components of the difference graph have to be taken into account, heuristics and approximate algorithms have to be investigated. For example, one could investigate the effect of preprocessing the graph database using a clustering algorithm. Additionally, the effect of using approximate frequent subgraph miners directly on the database of simple change graphs might improve the scalability of the solution. Furthermore, to reduce the amount of recommended \eo{s} the results could be postprocessed using heuristics (e.g., that the \eo{s} occur steadily over the modelling history).}{ An alternative approach, which we want to study in the future, is to use a clustering algorithm and then feed the clusters into the frequent subgraph mining step of our approach. This would allow us also to deal with examples in which the connected components are huge.}{} \par 
% TODO another example to show how powerful the approach could be
%One example just occurred to us while writing this paper: We are using separate .tex files for every section of the paper which are referenced in a main .tex file.
%Because we restructured the content of the sections we also renamed the .tex files of some sections. Unfortunately, the tool did not provide a ``renaming refactoring'' so we had to adjust the references in the main .tex file manually. 
%This is a operation that will occur in the tool and if it would have an explicit model and record the different states, it could learn these kind of operations or macros automatically and recommend them to the tool user. T




==> Content/discussion_original.tex <==
\section{Discussion}\label{sec:discussion}
\subsection{Research Questions}
%From the first two experiments, we can see from the high MAP@k values that \textsc{Ockham} is able to recover the \eo{s} that have been applied before. The third experiment shows that \textsc{Ockham} provides meaningful \eo{s} in a real-world setting. The observations from the first experiment suggest that the main driver for the performance of the frequent subgraph mining is the average number of nodes of our simple change graphs as well as the number of \eo{s} applied in the evolution steps yielding our model differences. To answer RQ 3, we have to take a closer look at the datasets for which our approach gives non-optimal results.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Answer to RQ 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \textbf{RQ 1: \textit{Is \textsc{Ockham} able to identify relevant \eo{s} in model repositories?}}
    We can answer this question with a ``yes''.
    Experiment 1 and 2 show high MAP scores. Only for a large number of applied operations and %according to Figure \ref{fig:eos_vs_components} also 
    a large size of the input graphs, \textsc{Ockham} fails in finding the applied \eo{s}. 
    We can see that our compression-based approach clearly outperforms the frequency-based approach used as a baseline.\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Answer to RQ 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \textbf{RQ 2: \textit{Is \textsc{Ockham} able to find typical edit operations or editing scenarios in a real-world setting?}}
    %Regarding scalability, we observed that for a too low support threshold of the frequent subgraph mining, the algorithms did not finish because there was not enough memory available. Increasing the threshold slightly, the algorithms typically finished in under 10 seconds. 
    The \eo{s} found by \textsc{Ockham} obtained significantly higher (mean/median) Likert scores than the random \eo{s}. Furthermore we observe a mean Likert score of almost 4.1. From this we can conclude that, compared to random ones, our mined \eo{s} can be considered as typical edit scenarios, on average. When looking at the mined \eo{s} it becomes clear, that \textsc{Ockham} is able to implicitly identify constraints, which where not made explicit in the meta-model. \inExtension{Also, except for one \eo{}, the mined \eo{s} appear in the sample dataset from experiment 4. }{}{}The \eo{s} recommended by \textsc{Ockham} are correct in most cases, and incomplete \eo{s} can be adjusted manually. We cannot state yet that the approach is also \emph{complete} (i.e., is able to find all relevant edit scenarios), though.\par
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Answer to RQ 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \textbf{RQ 3: \textit{What are the main drivers for \textsc{Ockham} to succeed or fail?}}
    %As we have seen from our first two experiments, the main indicators for a difficult dataset are the 
    From Table \ref{tbl:exp1_corr}, we observe that increasing the number of \eo{s} has a negative effect on the average precision. Increasing the perturbation has a slightly negative effect, which becomes stronger for a high number of applied \eo{s} and therefore %, according to figure \ref{fig:eos_vs_components}, 
    when huge connected components start to form. The number of differences $d$ (i.e., having more examples) has a positive effect on the rank, which is rather intuitive. 
    For the second experiment, from Table \ref{tbl:exp2_corr}, we can observe a strong dependency of the average precision on the perturbation parameter, which is, stronger than for the first experiment. On the other hand, the correlation to the number of applied \eo{s} is weaker.
\par To analyze the main drivers further, we take a deeper look into the results. We have to distinguish between the two cases that $(1)$ the correct \eo{} is not detected at all and $(2)$ the correct \eo{} has a low rank.% (i.e., appears later in the ranked list).

\textbf{Edit operation has not been detected:}
For the second experiment, in 22 out of 800 examples, \textsc{Ockham} was not able to detect both edit operations. In 10 of these cases the threshold has been set too high. To mitigate this problem, in a real-world setting, the threshold parameters could be manually adjusted until the results are more plausible. In the automatic approach, further metrics have to be integrated. 
%The threshold parameter could also be learned from other parameters, for instance, the average component size, number of components, or runtime of the mining up to some size of subgraphs. Another solution, more coherent with our viewpoint, is to evaluate the threshold based on the compression outcome, for example, the maximum compression found for the threshold.
\begin{table}[]
\centering
\caption{Main drivers for \textsc{Ockham} to fail in experiment 1.}
    \begin{tabular}{l|r r r r}
    \toprule
         &  &  \textbf{Mean} & &\\
         & \textbf{p} & \textbf{\#Nodes} & \textbf{Size at} & \textbf{Mining} \\
         & & \textbf{per comp} & \textbf{threshold} & \textbf{time} \\
    \midrule
   \textbf{Overall Mean} & $0.55$ & $57.6$ & $8.20$ & $1.26$ \\
    \begin{tabular}[l]{@{}l@{}} \textbf{Mean for un-} \\ \textbf{detected operation}\end{tabular} & $0.79$ & $109.0$ & $10.03$ & $2.55$\\
    
    \bottomrule
    
    \end{tabular}
\label{tbl:exp1_na_suspects}
\vspace{-1em}
\end{table}
Other factors that cause finding the correct \eo{s} to fail are the perturbation, average size of component, and the size at threshold, as can be seen from Table \ref{tbl:exp1_na_suspects}. Given a support threshold $t$, the \emph{size at threshold} is the number of nodes of the $t$-largest component. The intuition behind this metric is the following: For the frequent subgraph miner, in order to prune the search space, a subgraph is only allowed to appear in, at most, $t-1$ components. Therefore, the subgraph miner needs to search for a subgraph, at least, in one component with size greater than the \emph{size at threshold}. Usually, the component size plays a major role in the complexity of the subgraph mining. When the $t$-largest component is small, we could always use this component (or smaller ones) to guide the search through the search space and therefore we will not have a large search space. So, a large size of the component at threshold could be an indicator for a complicated dataset.\par
%We clearly see that perturbation, average size of a component, and the size at threshold are increased for the datasets for which our approach does not perform well. 
%Also, we can observe an increased time for the mining step for theses datasets.
%High perturbation and large connected components also cause that the correct subgraph does not or only rarely occurs isolated from other changes.
Looked deeper into the results of the datasets from the first experiment, for which the correct subgraph has not been identified, we can see that, for some of these subgraphs, there is a supergraph in our recommendations that is top-ranked. Usually this supergraph contains one or two additional nodes. Since we have a rather small meta-model, and we only use four other \eo{s} for the perturbation, it can happen rarely that these larger graphs occur with the same frequency as the actual subgraph. The correct subgraphs are then pruned away. 

%This is also one of the reasons why in the first experiment, the frequency approach performs slightly better. Since the size does not play a role here, the correct graphs could be ranked equal and have the chance to survive pruning.

%% Transient effects
%For the second experiment, the main issue is related to a too large support threshold. We observe problems especially for small $e$ and a large $p$. Some of the perturbations ``break up'' connected components (transient effects). This decreases the number of components containing an \eo{}. To understand these transient effects, we need to understand that the SCG resulting from the application of an \eo{} is not unique. For instance, preserved nodes of an \eo{} actually might have been created in the same model difference.

%If the left hand side of an \eo{} contains some elements which have been added by a previous \eo{} or which will be removed by another \eo{} in the same model difference $\Delta(m, i)$, we obtain a graph that is different from the graph obtained
%by just performing the \eo{} ``isolated'' from any other \eo{} application. This transient application of \eo{} can be handled by blowing up preserved nodes in the graphs, i.e., for a preserved node, we also add a node of type ``Add'' and a node of type ``Remove''. Further transient effects regarding right hand side nodes, we will not take into account here.

%If two \eo{s} are applied often together and depend on each other, they create a new ``effective'' operation. For example, the \eo{} of our running example in Figure \ref{fig:approach} can also be seen as two \eo{s}, one for adding the ports and connector and one for adding a new requirement. When these two \eo{s} appear frequently together, we will effectively see the combined \eo{}. The same can happen in a ``destructive'' manner, when an \eo{} is separated by the subsequent removal of some of its constituents. To mitigate these issues, the support threshold can be decreased (see above). We would then find more ``pure'' applications of the \eo{}.\par

\textbf{Edit operation has a low rank:}
%Note that a we observed a low rank (>5) only for the first experiment.
First, note that we observe a low rank (rank $\geq 5$) only very rarely. For the first experiment, it happened in 7 out of 2000 datasets, while for the second experiment, it did not happen at all. In Table \ref{tbl:exp1_low_rank_drivers}, we list the corresponding datasets and the values for drivers of a low rank. 
%For the datasets with rank $\geq 1$, the spearman correlation between the average precision and the average number of nodes per component is $-0.4$, and the one between average precision and the size at threshold is $-0.5$.
%Figure \ref{fig:exp1_low_rank_corr} shows a negative correlation between the average precision and the size at threshold as well as the average size of a component.
\begin{table}[]
\caption{Possible drivers for a low rank ($\geq 5$).}
\label{tbl:exp1_low_rank_drivers}
\begin{adjustbox}{center}
    \begin{tabular}{c c c r c l c}
    \toprule
         &  &  & \textbf{Mean} &  &  \\
       \textbf{d}  & \textbf{e} & \textbf{p} & \textbf{\#Nodes} & \textbf{Size at} & \textbf{Average} & \textbf{Rank} \\
        &  &  &  \textbf{per comp} & \textbf{threshold} & \textbf{precision} & \\
    \midrule
    $10$ & $92$ & $0.3$ & $142.2$ & $13$ & $0.13$ & $8$ \\
    $10$ & $67$ & $0.4$ & $91.0$ & $16$ & $0.14$ & $7$ \\
    $10$ & $78$ & $0.8$ & $87.3$ & $14$ & $0.14$ & $7$ \\
    $10$ & $98$ & $0.8$ & $127.7$ & $14$ & $0.067$ & $15$ \\
    $20$ & $81$ & $0.1$ & $227.0$ & $16$ & $0.13$ & $8$ \\
    $20$ & $99$ & $0.1$ & $272.2$ & $19$ & $0.010$ & $99$ \\
    $20$ & $100$ & $0.1$ & $272.7$ & $17$ & $0.013$ & $78$\\
 \bottomrule

    \end{tabular}
    \end{adjustbox}
\end{table}
%\begin{figure}[ht]
%			\centering
%			\includegraphics[width=\columnwidth]{pics/exp_1_bad_rank_corr.png}
%			\caption{Spearman correlation for average precision and possible drivers for a low rank in experiment 1 (rank $>1$).}
%			\label{fig:exp1_low_rank_corr}
%\end{figure}
One interesting observation is that, for some of the datasets with low-ranked correct subgraph, we can see that the correct graph appears very early in the subgraph lattice, for example, first child of the best compressing subgraph but rank $99$ in the output, or first child of the second best subgraph but rank $15$ in the output. This suggests that this is more a presentation issue, which is due to the fact that we have to select a linear order of all subgraph candidates for the experiment.\par
%The reason why our approach yields low rank for these datasets is the following:
%Many other (larger) subgraphs overlap with the subgraph containing the correct one. These are ranked higher using the compression metric (because they are bigger). So in this case, to present the results as a list sorted by compression is not the best approach. Instead, presenting the lattice directly or using some other way to present the results might be more suitable. One idea is, for example, to ``diagonally'' iterate over the lattice. In our examples it happens only rarely and we therefore leave the question of how to present the results as a future research question.

% TODO for the second experiment low rank only a few, but these ones we can catch with the optimal set (global) instead of the single eo approach.

%\subsubsection{Frequency vs. compression-based approach}

%For the frequency-based approach, we first sorted the list of subgraphs according to compression and then sorted according to frequency, that is, for the same frequency, the graphs will be sorted according to compression. This works well for the first experiment. For example, the first ranked \eo{} will be the most frequent subgraph, and there will be no bigger subgraph with the same frequency because it would have a larger compression, which contradicts our sorting. When the connected components become large (for a large $e$ parameter), subgraphs containing the correct subgraph but having a few additional nodes start to appear more frequently. Even though they appear less than or equal to the correct subgraph, they can have a higher compression, and in the end, using the compression based approach, will be pruned.
%This explains why the frequency-based approach works slightly better for the first experiment.
%Without compression-based sorting for graphs with the same frequency, the approach does not work at all. This can easily be understood 
%when we look at just the application of one \eo{}. In the SCG, we will have one connected component and all of the subgraphs have the same frequency. So, we need some other measure, for instance, related to the number of edges or the number of nodes, to select one of them. \par

%In the second experiment, some subgraphs of one (perturbed) \eo{} might appear with the same or a higher frequency than the other \eo{}. These subgraphs will be ranked higher by the frequency-based approach, which leads to a lower precision for these datasets.
In Experiment 3, we only found two mined \eo{s} that received an average Likert score below 3 from the five practitioners in the interviews.
The first one was a refactoring that was actually performed but that targeted only a minority of all models. Only two of the participants where aware of this refactoring, and one of them did not directly recognize it due to the abstract presentation of the refactoring. The other \eo{} that was also not considered as a typical edit scenario was adding a kind of document to another document. This \eo{} was even considered as illegal by 3 out of the 5 participants. The reason for this is the internal modeling of the relationship between the documents, which the participants were not aware of. So, it can also be attributed to the presentation of the results in terms of Henshin rules, which require an understanding of the underlying modeling language's meta-model.\par
For four of the \eo{s} of Experiment 3, some of the participants mentioned that the \eo{} can be extended slightly. We took a closer look at why \textsc{Ockham} was not able to detect the extended \eo{}, and it turned out that it was due to our simplifications of locality relaxation and also due to the missing type hierarchies in our graphs. For example, in one \eo{}, one could see that the fully qualified name (name + location in the containment hierarchy) of some nodes has been changed, but the actual change causing this name change was not visible, because it was a renaming of a package a few levels higher in the containment hierarchy that was not directly linked to our change. Another example was a ``cut off'' referenced element in an \eo{}. The reason why this has been cut off was that the element appeared as different sub-classes in the model differences and each single change alone was not frequent.\par

To summarize: The main drivers for \textsc{Ockham} to fail are a large average size of components and the size at threshold. The average size is related to the number of \eo{s} applied per model difference. In a practical scenario, huge differences can be excluded when running \eo{} detection. The size of the component at threshold can be reduced by increasing the support threshold parameters of the frequent subgraph mining. With higher threshold, we increase the risk of missing some less frequent \eo{s}, but the reliability for detecting the correct (more frequent) operations is increased. Having more examples improves the results of \textsc{Ockham}.
    %So this is a trade-off we have to do. Rerunning the algorithm with different choices for the threshold parameter will increase the chance of detecting the best set of \eo{s}. This can also be used in combination with a genetic algorithm and the target to maximize the global compression, which we leave for future research.
    
    \textbf{RQ 4: \textit{What are the main parameters for the performance of the frequent subgraph mining?}}
     From Table \ref{tbl:exp1_corr}, we can observe a strong Spearman correlation of the mining time with the number of applied \eo{s} $e$ ($0.89$) and implicitly also the average number of nodes per component ($0.83$). If we only look at \eo{s} with rank $> 1$, we observe a strong negative correlation of $-0.51$ with the average precision (not shown in Table \ref{tbl:exp1_corr}). This actually means that large mining times usually come with a bad ranking. The same effect can be observed for Experiment 2 (Table \ref{tbl:exp2_corr}). We can also see, that the mining time correlates with the size at threshold.


%In figure \ref{fig:aps}, we list the average precision depending on our control parameters $e$ and $p$ (we fixed $d=10$ for this experiment). 
% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=\columnwidth]{pics/exp2-AP-eos-perturbation.png}
% 			\caption{The average precicions for the second experiment, number of \eo{s} on the x-axis and perturbation on the y-axis.}
% 			\label{fig:aps}
% \end{figure}

% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=\columnwidth, trim= 20 60 30 60, clip]{pics/exp2-correlations.png}
% 			\caption{The Spearman correlation matrix for the second experiment.}
% 			\label{fig:exp2_corr}
% \end{figure}

%Since the computational complexity of embedding all the frequent subtrees is very high, we only look at the top-$N$ trees. 
%For the order of the trees, we will compare the following two approaches:

%\begin{itemize}
%    \item Iterating through the trees ordered by tree compression $cr(t) = ({\operatorname{supp}}(t)-1) \cdot (2|V_t|-1)$.
%    \item Firstly, performing non-dominated sorting\footnote{We borrow this idea from the NSGA-II genetic algorithm (\cite{Deb2000}).} with the two objectives \textit{support} and \textit{number of nodes}. And secondly, iterating through the non-dominated fronts of this sorting by starting at the most frequent trees and going through the front to the largest trees and then jumping again to the most-frequent trees in the next front.
%\end{itemize}

%We stop the iteration as soon as we found $N$ frequent (i.e., support greater than some threshold $T$) induced subgraphs.

%As another technique, to reduce the number of trees, we experiment using a diversity sampling strategy. 

%For some integer $D$, we sample D trees with the largest minimal node label distance $d$. Since this is again a computationally intensive problem, we use some approximate algorithm for the sampling. Due to space constraints, we omit the details of this sampling here.
\inExtension{
\textbf{RQ~5: \textit{What is the practical impact of the \eo{s} discovered by \textsc{Ockham} in the context of the case study in \secref{sec:case-study}?}}
In experiment 4, we lifted the changes using the \eo{s} discovered by \textsc{Ockham} and applied the classification into refactorings and critical \eo{s}.
From this experiment we can see, first of all, that our \eo{s} also occur in practice. There is only one \eo{} that did not occur at all in our example models. The reason is that this \eo{} corresponds to a one-time refactoring that was done some time ago, but was not included in our randomly selected sample. Furthermore, the \eo{s} mined by \textsc{Ockham} can be used to compress model differences significantly. 
Since they are also meaningful to domain experts (see RQ~2), they can be used to summarize model differences. 
Rather ``small'' changes, for example, adding a package ($\sim23\%$ of the change sets) or renaming a property ($\sim10\%$ of the change sets), occur with a much higher frequency than more complex \eo{s} such as adding an external port with multiplicities ($\sim1.3\%$ of the change sets). In general, from the results of experiment 4, we can see that critical \eo{s} are more rare compared to refactoring \eo{s}. On the other hand, they provide a higher compression of the model differences. The classification of the \eo{s} could also be used to filter out irrelevant changes in the analysis of model differences. Nevertheless, the classification is most likely task-dependent and we cannot be sure that this observation also holds for other classifications.\par
Furthermore, the the distribution of \eo{s} in a model difference can tell us something about the nature of the evolution step. For example, we can determine ``hot spots'', where a lot of critical \eo{s} are performed.\par
Even though we did not evaluate the semantic lifting approach in a long-term application, engineers at \partner{} support the hypothesis that it can be useful for \sple{} related tasks and quality assurance of models. Overall, we can conclude that the \eo{s} discovered by \textsc{Ockham} can be useful in the context of the case study in \secref{sec:case-study}.
}{}{
}
\inExtension{
\begin{tcolorbox}[arc=0pt,outer arc=0pt, boxrule=0pt, breakable,  sharpish corners,enhanced, drop lifted shadow]
In Summary, \textsc{Ockham} is able to identify relevant \eo{s} that correspond to typical edit scenarios in the history of projects. The mining doesn't scale to large connected model differences, so these have to be excluded from the mining. As a consequence of this, but also because a minimum frequency threshold has to be set, we can not claim that our approach is \emph{complete} in the sense that it will discover all relevant \eo{s}. Furthermore, hard tasks for the subgraph miner typically lead also to bad results with respect to the correctness of the mined \eo{s}. The \eo{s} discovered by \textsc{Ockham} can also be applied in practical application scenarios, for example, to ease the analysis of large model differences by employing semantic lifting and filtering.
\end{tcolorbox}
}{}{}
% Change profiles
\inExtension{
\subsection{Further applications} \label{sec:addapplications}
We made an interesting observation when analyzing the distribution of the \eo{s} in the fourth experiment (see \figref{fig:change_profiles}). Between some of the sample model differences, we observe high similarities of their distributions, while for between others, there is almost no correlation. In other words, we can see clusters of the \eo{} distributions, which can be seen more easily in \figref{fig:change_profile_correlation}. 

\begin{figure*}[ht]
			\centering
			\includegraphics[clip, trim=0cm 8.5cm 0cm 8.5cm,width=.8\textwidth]{pics/change_profile_correlation.pdf}
			\caption{Pearson correlation of the \eo{} frequency distributions for 40 sample model differences. We have removed a dominant \eo{} (Adding a {\sf Package}) from the distributions to make the clusters appear more clearly in this visual representation. Qualitatively, the same clusters will be obtained though, without removing this \eo{} from the frequency distribution.}
			\label{fig:change_profile_correlation}
\end{figure*}

A closer look at these clusters reveals that there is indeed a similarity in the model differences. 
For example, the cluster $[11-15, 17-23, 25-26]$ contains a lot of functional modifications of the models. For example, interfaces have been changed, so called {\sf Functional Addresses} have been added, and activity diagrams were modified. The cluster $[24, 31-33]$ also contains functional modifications, but additionally documentation has changed a lot. For example, so called {\sf Reference Documents} have been added, system requirements have been added or changed, and comments were added or changed. The cluster $[6-10, 27]$ contains a lot of added functionality but less modification to the documentation. Furthermore, the change profiles between different submodels for the same trainset type are often very similar. We can also find some model differences that are quite different from all other model differences and play some special role, for example, for cross-cutting functionality like test automation. \par
This suggests that the \eo{s} frequency distributions can be seen as a kind of \emph{change profile} for the model difference, which can be used, for example, to gain further insights into the model differences. These change profiles can be used to reason about model differences or model evolution from a high-level perspective. Insights about the clusters can also be used, for example, to detect uncommon and possibly undesired changes.
Since they are probability distributions, methods from statistics can be applied. Furthermore, they can also be seen as normed vectors (w.r.t. the $1$-norm) and therefore also methods from linear algebra can be applied to further analyze model differences.
Besides the analysis of the model evolution, the change profile can also be used for simulating model evolution, especially if different evolution scenarios are to be investigated. Similar profiles have already been used for model evolution simulation, for example, by \cite{Heider2010}, who refer to the profiles as evolution profiles. Another statistical approach to model simulation based on semantic lifting has been proposed by \cite{Yazdi2016} but their \eo{s} have to be defined manually. \par
Dual to this cluster analysis, the change profiles can also be used to analyze co-occurrences of \eo{s}. For example, we observe a large Pearson correlation of~$\sim0.99$ between the \eo{s} {\sf ChangeUseCase} and {\sf ChangeActivity}. This could also indicate that these \eo{s} can be combined to form a new, larger \eo{}, which is the case in this concrete example. Some of the \eo{s} seem to be almost uncorrelated, for example, we observe that adding new functionality rarely occurs together with modifying existing functionality. Similar co-evolution analysis have been investigated in detail by \cite{getir2018supporting}. Note that \textsc{Ockham} is also a kind of co-change analysis that also takes structural similarities into account. The interplay between statistical co-occurrence analysis and structural graph mining in the analysis of model evolution is a promising future research direction.
}{}{}


% Limitations
\subsection{Limitations} \label{sec:limitations}
% locality relaxation
\textit{Locality relaxation:}
One limitation of our approach is the locality relaxation, which limits our ability to find patterns that are scattered across more than one connected component of the simple change graph. As we have seen in our railway case study, this usually leads to incomplete \eo{s}.
% If elements that have something to do which each other are not connected in the model, this is a shortcoming of the model but in practise it can be observed. => Not always, e.g. fqn chnged because super package renamed (transitive changes and derived properties)
Another typical example for violating the relaxation are naming conventions.
%For example, in out example meta-model ``Simple Component Model'', we could omit the directly link between the requirement and the component and instead link them via an attribute name. 
%This kind of additional context can not yet be learned. When the context is known, it can be added to the meta-model and the instances can be automatically augmented by the additional context. 
In the future, we plan to use natural language processing techniques such as semantic matching to augment the models by further references. 
%(or edges in the graph). 
%based on seman case this kind of context should also be learned from the models, more sophisticated approaches are possible. One idea is, to use natural language processing to create additional links between model elements based on their textual semantic similarity. 
\par
% No attribute information is used
\textit{No attribute information:}
For our experiments, we did not take attribute information into account. Attributes (e.g., the name of a component) could also be integrated into the \eo{} as preconditions or to extract the parameters of an \eo{}. 
%Furthermore, some attribute value changes could be derived. 
For the purpose of summarizing a model difference or identifying violations in a model difference, preconditions and parameters are not important, though, but only the presence of structural patterns. 
%In case a violation is only a violation under certain attribute preconditions, these could be added manually.\par

% Model features
\textit{Application to simplified graphs:}
Generally, an \eo{} is a model transformation. Model transformation engines such as \textsc{Henshin} provide features to deal with class inheritance or multi-object structures (roughly speaking, foreach loops in model transformations). In our approach, we are not leveraging these features yet. 
They could be integrated into \textsc{Ockham} in a post-processing step. 
%For example, if two rules are discovered, which are identical except that one child class is replaced by another child class of some parent class, we can deduce that in the \eo{} the child classes can be replaced by the parent class.
For example, one possibility would be to feed the example instances of patterns discovered by \textsc{Ockham} into a traditional MTBE approach~\citep{Kehrer2017}. 
%Negative examples can be collected at runtime by user feedback but this is not of our concern here because for our use case application- and non-application conditions can be ignored.
\par
% transient effects
\textit{Transient effects:}
We do not take so-called transient effects into account yet. One applied \eo{} can invalidate the pre- or post-conditions of another \eo{}. 
%We believe, though, that \textsc{Ockham} should be able to cope with these effects already, and 
However, we have seen in our experiments that this only causes problems in cases where we apply only a few ``correct'' \eo{s} with high perturbation. In a practical scenario, the ``perturbations'' will more likely cancel each other out.
%When the transient effects happen only rarely, it is still possible to discover the original operations. 
When a transient effect occurs very frequently, a new pattern will be discovered. That is, when two (or more) operations are always applied together, we want to find the composite pattern, not the constituent ones.\par  
% Jitter and local compression only
\textit{Focus on single subgraphs instead of sets:}
Another limitation is the fact that we focused the optimization on \emph{single} \eo{s} but not a \emph{complete set} of \eo{s}. 
One could detect only the most-compressing \eo{} and then substitute this in the model differences and re-run the mining to discover the second most-compressing \eo{} and so on. Another solution would be to detect a set of candidate \eo{s} using \textsc{Ockham} and then select an optimal set 
using a meta-heuristic search algorithm optimizing the \emph{total compression}. % as well as minimizing the elements in the model differences that are not covered by an \eo{}.
We leave this for further research.\par
% Since we haven't decomposed our model differences yet by the discovered \eo{s}, some of them might overlap and ``contradict'' each other. Therefore, the computed list of \eo{s} is a set of recommendations and needs to be further analyzed by a domain expert. For future research, we plan to compute the best set of \eo{s} (i.e., the compression maximizing set $SG$ in the language of SCGs) instead of single \eo{s}, which would solve this overlapping problem. A genetic algorithm as used by Mokaddem et al. \cite{Mokaddem2018} can be used for this task.
\inExtension{\textit{Completeness of the set of mined \eo{s}:}
As we can see from experiment 4, a set of 30 \eo{s} is still far from being complete. In fact, with this set, we missed $70\%$ of changes in our sample model differences. Anyway, the approach can also be applied iteratively, in the sense that \eo{s} which are already approved by domain experts can be used to substitute the corresponding subgraph by a single node. The graph mining can then be applied on these \emph{contracted} graph databases until all changes are included in a change set.  However, since a change does not unambiguously belong to a change set, this approach would be subject to the limitation from the previous paragraph.
%In the end, the set of \eo{s} might not be consistency-preserving and not complete (see also \cite{Kehrer2011}), i.e., we can not completely decompose every model difference in terms of the \eo{s} we have discovered. Also, we have to set the support threshold for the subgraph mining to be able to find the least frequent \eo{} that we want to discover. This will create some kind of ``jitter'' for the more frequent subgraphs. I.e., we will also identify perturbations of some operations and some of the perturbations possibly having a better compression value than other \eo{s}. This will in the end lead to a non-optimal ranking for these other operations.
%We see two possible solutions for this limitation. 
}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THREATS TO VALIDIDY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Threats to Validity}\label{sec:threats}
%Construct validity
%\textit{Construct validity:}
\textit{Internal validity:}
We have designed the first two experiments such that we can control input parameters of interest and observe their effect on the outcome. \textsc{Ockham} makes assumptions such as the locality relaxation, which could impair real-world applicability. Because of this and since we can not claim that the results from the first two experiments also hold true in a real-world setting, we additionally applied \textsc{Ockham} to an industrial case study. Our results increase our confidence that \textsc{Ockham} also gives reasonable results in a practical scenario.\par
%Internal validity
%\textbf{Internal validity:}
In our simulations, we applied the \eo{} randomly to a meta-model. To reduce the risk of observations that are only a result of this sampling, we created many example models. In the real-world setting, we compared the mined edit operations to random ones to rule out ``patternicity'' \citep{shermer2008patternicity} as an explanation for high Likert rankings. None of our participants reported problems in understanding \textsc{Henshin}'s visual notation, which gives us confidence regarding their judgements (despite for misconceptions). 
\changed{The participants of the interviews in the third experiment were also involved in the project where the model history was taken from. There might be the risk that the interviewees have only discovered operations they have ``invented''. In any case, because of the huge project size and because 22 out of 25 of the edit operations were recognized as typical by more than one of the participants, this is unlikely.}\par
% External Validity: 
\textit{External validity:}
Some of the observations in our experiments could be due to the concrete set of \eo{s} in the example or even due to something in the meta-models. In the future, \textsc{Ockham} has to be tested for further meta-models to increase the external validity of our results. We have validated our approach in a real-world setting, which increases our confidence in its practicality, though. \inExtension{As can be seen from experiment 4, with the set of 30 \eo{s}, $70\%$ of the changes are not part of a change set. It is therefore not yet clear, if the results regarding the compression of model differences also hold true when using larger sets of \emph{meaningful} \eo{s}.}{}{}
Since we have used an exact subgraph miner, we can be sure that the discovered \eo{} are independent of the subgraph mining algorithm. 
%Regarding the performance of the mining, we should also consider other miners. We also experimented with gSpan and DIMSpan and for our simulations, \textsc{Gaston} worked best but we didn't perform a quantitative comparison of different subgraph mining algorithms. 
\par

==> Content/experiments_old.tex <==

In this section, we will evaluate our approach in two controlled experiments and one real-world industry case study in the railway domain.

\subsection{Research Questions}
We evaluate \textsc{Ockham} w.r.t.\ the following research questions:
\begin{itemize}
     
\item \begin{bfseries} RQ 1: \end{bfseries}  \textit{Is \textsc{Ockham} able to identify \eo{s} that have actually been applied in model repositories?} If we apply some operations to models, \textsc{Ockham} should be able to discover these from the data. Furthermore, when different \eo{s} are applied and overlap, it should still be possible to discover them.
    %\item \begin{bfseries} Research Question 2 - \end{bfseries}  How does approximate mining compare to exact frequent subgraph mining?
    
\item \begin{bfseries} RQ 2: \end{bfseries} \textit{Is \textsc{Ockham} able to find typical \eo{s} or editing scenarios in a real-world setting?} Compared to the first research question, \textsc{Ockham} should also be able to find typical scenarios in practice for which we do not know which operations have been actually applied to the data. Furthermore, it should be possible to derive these \eo{s} in a real-world setting with large models and complex meta-models.
    
\item \begin{bfseries} RQ 3: \end{bfseries} \textit{What are the main drivers for \textsc{Ockham} to succeed or fail?} We want to identify the characteristics of the input data or parameters having a major influence on \textsc{Ockham}.
    
\item \begin{bfseries} RQ 4: \end{bfseries} \textit{What are the main parameters for the performance of the frequent subgraph mining?} Frequent subgraph mining has a very high computational complexity for general cyclic graphs. We want to identify the characteristics of the data in our setting that influence the mining time.

\inExtension{
\item \begin{bfseries} RQ 5:\end{bfseries}   \textit{What is the practical impact of the \eo{s} discovered by \textsc{Ockham} in the context of the case study introduced in \secref{sec:case-study}?} One of our main motivations is to compress differences in our case study of \secref{sec:case-study}. We evaluate which degree of compression our mined operations provide in this scenario.
}{}
\end{itemize}


\changed{For RQ 1, we want to rediscover the \eo{s} from our ground truth, whereas in RQ 2, the discovered operations could also be some changes that are not applied in ``only one step'' but appear to be typical for a domain expert. We refer to both kinds of change patterns as ``meaningful'' \eo{}.}

\subsection{Experiment Setup}
We conduct \inExtension{four}{three}{} experiments to evaluate our approach. In the first two experiments, we run the algorithm on \changed{synthetic model repositories}. We know the ``relevant \eo{s}'' in these repositories, since we define them, and apply them to sample models. We can therefore use these experiments to answer RQ 1.
Furthermore, since we are able to control many properties of our input data for these simulated repositories, we can also use them to answer RQ 3 and RQ 4. In the third experiment, we apply \textsc{Ockham} to the dataset from our case study presented in \secref{sec:case-study} to answer RQ 2. \changed{The first two experiments help us to find the model properties and the parameters the approach is sensible to. Their purpose is to increase the \emph{internal validity} of our evaluation. To increase \emph{external validity}, we apply \textsc{Ockham} in a real-world setting as well. None of these experiments alone achieves sufficient internal and external validity~\citep{siegmund2015views}, but the combination of all experiments is suitable to assess whether \textsc{Ockham} can discover relevant \eo{s}.} 
\inExtension{
In the fourth experiment, we use the \eo{s} from the third experiment to semantically lift the low-level differences using the approach of \cite{Kehrer2011}. We then compute the compression ratio on a sample of model differences to answer RQ~5.
}{}{}
%All data and scripts to execute experiment 1 and 2 are provided within our replication package.
%MR@k is the mean over all graph databases for the fractions of correct graphs among the first $k$ in the ranked list divided by the number of relevant graphs and
%MAP@k is the mean over all graph databases of the weighted (by reciprocal rank) average of the precisions up to rank $k$. MAP@k therefore penalizes lower ranked matches.

%To given an example for these metrics, suppose we apply one \eo{} and our algorithm outputs exactly this \eo{} at the first rank for all datasets. In this case $MR@1 = MR@k = 1 = MAP@1 = MAP@k$. If we apply two \eo{s} and our algorithm finds them at positions two and three, for all of our datasets, then $MR@1 = 0$, $MR@2 = 0.5$, and $MR@3 = MR@k = 1$. In this case MAP@k penalizes the lower ranks (perfect would be first and second rank) and we have $MAP@1 = 0$, $MAP@2 = 0.25$, and $MAP@3 = MAP@k = 0.75$.
%\begin{remark}
%There exist some variations of these definitions in the recommender systems and information retrieval literature.
%\end{remark}

We run the experiments on an Intel Core™ i7-5820K CPU @ 3.30GHz × 12 and 31.3 GiB RAM. For the synthetic repositories, we use 3 cores per dataset.

\textbf{Experiment 1:}
As a first experiment, we simulate the application of \eo{s} on a simple component model. The meta-model is shown in \figref{fig:difference-graph}.\par
For this experiment, we only apply one kind of \eo{} (the one from our running example in \figref{fig:approach}) to a random model instance. The Henshin rule specifying the operation consists of a graph pattern comprising 7 nodes and 7 edges. We create the model differences as follows:
We start with an instance $m_0$ of the simple component meta-model with 87 {\sf Packages}, 85 {\sf Components}, 85 {\sf SwImplementations}, 172 {\sf Ports}, 86 {\sf Connectors}, and 171 {\sf Requirements}.
%This size corresponds to the typical size of a (sub-)model of our real-world dataset.
Then, the \eo{} is randomly applied $e$ times to the model %(we randomly choose a match of the LHS of the \eo{}) 
obtaining a new model revision $m_1$. This procedure is applied iteratively $d$ times to obtain the model history
%\begin{equation*}
   $m_0 \xrightarrow[]{} m_1 \xrightarrow[]{} \dots m_{d - 1} \xrightarrow[]{} m_{d}.$
%\end{equation*}
Each evolution step $m_i \xrightarrow[]{} m_{i+1}$ yields a difference $\Delta(m_i,m_{i+1})$.
\par
Since we can not ensure completeness of \textsc{Ockham} (i.e., it might not discover all \eo{s} in a real-world setting), we also have to investigate how sensible the approach is to undiscovered \eo{s}. Therefore, to each application of the \eo{}, we apply a random perturbation. More concretely, a perturbation is another \eo{} that we apply with a certain probability $p$. This perturbation is applied such that it overlaps with the application of the main \eo{}. % (i.e., the actual \eo{} and the perturbation \eo{} have some nodes in common). 
We use the tool \textsc{Henshin} \citep{Biermann2012} to apply model transformations to one model revision.
We then build the difference of two successive models as outlined in \secref{sec:appraoch}. 
In our experiment, we control the following parameters for the generated data. 

\begin{itemize}
    \item $d$: The number of differences in each simulated model repository. For this experiment, $d \,\in\, \lbrace10,20 \rbrace$.
    \item $e$: The number of \eo{s} to be applied per model revision in the repository, that is, how often the edit operation will be applied to the model. For this experiment, $e \,\in\, \lbrace 1, \dots , 100\rbrace$.
    \item $p$: The probability that the operation will be perturbed. For this experiment, we use $p \in \lbrace 0.1, 0.2, \dots, 1.0 \rbrace$.
\end{itemize}

This gives us 2000 ($= 2\times100\times10$) datasets for this experiment. A characteristics of our datasets is that, increasing $e$, the probability of changes to overlap increases, as well. Eventually, adding more changes even decreases the number of components in the SCG while increasing the average size of the components. %(see Figure \ref{fig:eos_vs_components})
\par
\textsc{Ockham} suggests a ranking of the top $k$ subgraphs (which eventually yield the learned edit operations). In the ranked suggestions of the algorithm, we then look for the position of the ``relevant \eo{}'' by using a graph isomorphism test.
%Table \ref{tbl:exp1-runtime}
%The reason to use only small values for the perturbation parameter is that some of the perturbations cause a split in the connected components and for to large $p$, the relative threshold of $0.4$ is to big to detect the correct \eo{}.
% \begin{table}[]
% \begin{tabular}{|
% >{\columncolor[HTML]{EFEFEF}}l |l|l|l|l|
% >{\columncolor[HTML]{34CDF9}}l |}
% \hline
% {\color[HTML]{000000} } &
%   \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}$\varnothing $ nb. nodes\\ per comp\end{tabular} &
%   \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} e} &
%   \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}size at \\ threshold\end{tabular}} &
%   \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}AP\end{tabular}} &
%   \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} p} \\ \hline
% Mining time &
%   \cellcolor[HTML]{FD6864}0.78 &
%   \cellcolor[HTML]{FD6864}0.79 &
%   \cellcolor[HTML]{DAE8FC}-0.17 &
%   \cellcolor[HTML]{3166FF}-0.21 &
%   \cellcolor[HTML]{DAE8FC}-0.08 \\ \hline
% % \begin{tabular}[c]{@{}l@{}}$\varnothing $ nb. nodes\\ per comp.\end{tabular} &
% %   - &
% %   \cellcolor[HTML]{FE0000}0.99 &
% %   \cellcolor[HTML]{DAE8FC}-0-07 &
% %   \cellcolor[HTML]{3166FF}-0.24 &
% %   -0.14 \\ \hline
% % e &
% %   - &
% %   - &
% %   \cellcolor[HTML]{34CDF9}-0.11 &
% %   \cellcolor[HTML]{3166FF}-0.22 &
% %   -0.09 \\ \hline
% % \begin{tabular}[c]{@{}l@{}}size at \\ threshold\end{tabular} &
% %   - &
% %   - &
% %   - &
% %   \cellcolor[HTML]{34CDF9}-0.12 &
% %   -0.15 \\ \hline
% % \begin{tabular}[c]{@{}l@{}}AP\end{tabular} &
% %   - &
% %   - &
% %   - &
% %   - &
% %   \cellcolor[HTML]{FFCCC9}0.06 \\ \hline
% \end{tabular}
% \caption{Spearman correlations for the mining time for fixed relative threshold $0.4$ and $p \leq 0.4$.}
% \label{tbl:exp1-runtime}
% \vspace{-1em}
% \end{table}
% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=\columnwidth, trim= 20 100 80 60, clip]{pics/exp1_runtime.png}
% 			\label{fig:exp1_runtimes}
% 						\caption{Spearman corrleations for the first experiment for fixed relative threshold $0.4$ and $p \leq 0.4$.}
% \end{figure}
To evaluate the ranking, we use the ``mean average precision at k'' (MAP@k), which is commonly used as an accuracy metric for recommender systems~\citep{schroder2011setting}:
% \begin{equation*}
%     MR@k := \frac{1}{|D|} \sum_{\text{D}} \frac{|\text{relevant subgraphs up to rank k}|}{|\text{total relevant subgraphs}|}\text{,} 
% \end{equation*}
% and
\begin{equation*}
\operatorname{MAP@k} := \frac{1}{|D|} \sum_{\text{D}} \operatorname{AP@k} \, \text{,}
\end{equation*}
% \begin{equation*}
% \begin{aligned}
% \operatorname{AP@k} &:= \frac{\sum_{i=1}^{k} \operatorname{P}(i) \cdot \operatorname{rel}(i)}{{|\text{total relevant subgraphs}|}} \, \text{, and} \\
% \operatorname{MAP@k} &:= \frac{1}{|D|} \sum_{\text{ds} \in \text{D}} \operatorname{AP@k} \, \text{,}
% \end{aligned}
% \end{equation*}
where $D$ is the family of all datasets (one dataset represents one repository) and AP@k is defined by 
\begin{equation*}
\operatorname{AP@k} := \frac{\sum_{i=1}^{k} \operatorname{P}(i) \cdot \operatorname{rel}(i)}{{|\text{total set of relevant subgraphs}|}} \, \text{, } 
\end{equation*}
where P($i$) is the precision at $i$, and rel($i$) indicates if the graph at rank $i$ is relevant. 
%MR@k is the mean over all graph databases for the fractions of correct graphs among the first $k$ in the ranked list divided by the number of relevant graphs and
%MAP@k is the mean over all graph databases of the weighted (by reciprocal rank) average of the precisions up to rank $k$. MAP@k therefore penalizes lower ranked matches.

%To given an example for these metrics, suppose we apply one \eo{} and our algorithm outputs exactly this \eo{} at the first rank for all datasets. In this case $MR@1 = MR@k = 1 = MAP@1 = MAP@k$. If we apply two \eo{s} and our algorithm finds them at positions two and three, for all of our datasets, then $MR@1 = 0$, $MR@2 = 0.5$, and $MR@3 = MR@k = 1$. In this case MAP@k penalizes the lower ranks (perfect would be first and second rank) and we have $MAP@1 = 0$, $MAP@2 = 0.25$, and $MAP@3 = MAP@k = 0.75$.
%\begin{remark}
%There exist some variations of these definitions in the recommender systems and information retrieval literature.
%\end{remark}
For this experiment, the number of relevant \eo{s} (or subgraphs to be more precise) is always one. Therefore, we are interested in the rank of the correct \eo{}. Except for the case that the relevant \eo{} does not show up at all, MAP@$\infty$ gives us the mean reciprocal rank and therefore serves as a good metric for that purpose.

For comparison only, we also compute the MAP@k scores for the rank of the correct \eo{s} according to the frequency of the subgraphs. Furthermore, we investigate how the performance of subgraph mining depends on other parameters of \textsc{Ockham}. We are also interested in how average precision (AP), that is, AP@$\infty$, depends on the characteristics of the datasets. Note that for the first two experiments, we do not execute the last canonical step of our approach (i.e., deriving the \eo{} from a SCG), but we directly evaluate the resulting subgraph from Step~4 against the simple change graph corresponding to the \eo{}.\par

To evaluate the performance of the frequent subgraph miner on our datasets, we fixed the relative threshold (i.e., the support threshold divided by the number of components in the graph database) to $0.4$. We re-run the algorithm for this fixed relative support threshold and $p \leq 0.4$.

\textbf{Experiment 2:}
In contrast to the first experiment, we want to identify in the second experiment more than one \eo{} in a model repository. We therefore extent the first experiment by adding another \eo{}, applying each of the operations with the same probability. To test whether \textsc{Ockham} also detects \eo{s} with smaller compression than the dominant (in terms of compression) \eo{}, we choose a smaller second operation. The Henshin rule graph pattern for the second operation comprises 4 nodes and 5 edges. \changed{It corresponds to adding a new {\sf Component} with its {\sf SwImplementation} and a {\sf Requirement} to a {\sf Package}}.\par 
Since the simulation of model revisions consumes a lot of compute resources, we fixed $d=10$ and considered only $e<=80$ for this experiment. The rest of the experiment is analogous to the first experiment.

\textbf{Experiment 3:}
The power of the simulation to mimic a real-world model evolution is limited. Especially, the assumption of random and independent applications of \eo{s} is questionable.
Therefore, for the third experiment, we use a real-world model repository from the railway software development domain (see \secref{sec:case-study}). For this repository, we do not know the operations that have actually been applied. We therefore compare the mined \eo{s} with \eo{s} randomly generated from the meta-model, and want to show that the mined \eo{s} are significantly more ``meaningful'' than the random ones.\par
\inExtension{The models in this case are SysML models in MagicDraw but there is an EMF export of the SysML models, which we can use to apply our toolchain. %The entire model has been split into several sub-models. 
%The modeling history of each model is maintained on a TeamWork server. 
%There is not only a temporal history, but also a spatial dimension, since every sub-model has an instance for multiply trainset platforms (i.e., different train types). E.g., for the HVAC, there is a branch for the high-velocity train or the high-capacity train. 
%The MagicDraw models are transformed to a domain specific model which has many similarities to SysML. For this domain specific model, there is an EMF Ecore meta-model. We can therefore easily apply our approach to the transformed MagicDraw models.
}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some statistics on the differences
For this experiment, we mined
% (i.e., a difference in time). 
546 pairwise differences, with 4109 changes, on average, which also contain changed attribute values (one reason for that many changes is that the engineering language has changed from German to English). The typical model size in terms of their abstract syntax graphs is 12081 nodes; on average, 50 out of 83 meta-model classes are used as node types. 
% IN PHD Thesis, also add more details on the datasets and graphs. Mention the problem of meta-model changes which makes the mining very difficult and that we don't took all revisions into account in our case (but which is not important for this study).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Our dataset includes the successive differences across all sub-models and all trainset platforms.
\par
To evaluate the quality of our recommendations, we conducted a semi-structured interview with five domain experts of our industry partner: 2 system engineers working with one of the models, 1 system engineer working cross-cutting, 1 chief system architect responsible for the product line approach and the head of the tool development team. We presented them 25 of our mined \eo{s} together with 25 \eo{s} that were randomly generated out of the meta-model. The \eo{s} were presented in the visual transformation language of \textsc{Henshin}, which we introduced to our participants before. On a 5-point Likert scale, \changed{we asked whether} the \eo{} represents a typical edit scenario (5), is rather typical (4), can make sense but is not typical (3), is unlikely to exist (2), and does not make sense at all (1). We compare the distributions of the Likert score for the population of random \eo{s} and mined \eo{s} \changed{to determine whether the mined operations are typical or meaningful}. \par
In addition, we discussed the mined \eo{s} with the engineers that have not been considered to be typical. %edit scenarios. 

%We also asked the participants, if presenting the model difference in terms of typical \eo{s} can help understanding the model difference and support model merging or other tasks in Model-Driven Engineering.
\inExtension{
\textbf {Experiment 4:}
Higher-level \eo{s} typically comprise several more fine-grained edit steps. 
\cite{Kehrer2011} presented an approach that allows to represent a model difference in terms of previously defined \eo{s}. Changes in the model difference that belong to the application of one \eo{} are grouped together in a \emph{lifted model difference}. A group of changes that belong to the application of one \eo{} is called a \emph{change set}. Using this lifting approach, we can evaluate to what extend the \eo{s} mined by \textsc{Ockham} can compress model differences.
For this, in the fourth experiment, we use the 25 mined \eo{s} from the third experiment and five additional \eo{s} discovered by \textsc{Ockham} for a semantic lifting of a sample of 40 model differences from our industrial scenario from \secref{sec:case-study}. More concretely, we randomly select 40 submodels in their current revision and compute the difference between this revision and 25 revisions earlier of the same submodel. If no 25 revisions are available, we compute the difference to the earliest possible revision. Of course, our 30 \eo{s} are not yet complete, that is, some changes will be missed. We will therefore not only report the total compression ratio but also the relative compression ratio (i.e., the compression ratio with respect to the changes that are covered by the 30 \eo{s}).
We define the compression ratio as follows:

\begin{equation*}
\operatorname{c} := \frac{{|\text{changes before lifting}|}}{|\text{change sets}| + |\text{ungrouped changes}|}\,, 
\end{equation*}
where by \emph{ungrouped changes} we refer to changes that are not included in any of the change sets after the semantic lifting.
Similarly, the relative compression ratio is defined as:

\begin{equation*}
\operatorname{c_{rel}} := \frac{{|\text{changes before lifting}| - |\text{ungrouped changes}|}}{|\text{change sets}|}
\end{equation*}

With the help of the domain experts we furthermore divided the set of 30 \eo{s} into two subsets. One subset contains refactorings like renaming operations or move operations, while the other subset contains \eo{s} which represent important functional evolution. We will refer to the second subset as \emph{critical \eo{s}}. 22 \eo{s} have been classified as critical and 8 as refactorings. We will also report the compression ratio for these critical operations separately. The reason for this separate reporting is that for some of the tasks related to model differences, refactoring is less relevant and can be ignored, while the critical \eo{s} are crucial for the analysis. An example for such a task is the analysis of the functional changes of a product between two successive software qualifications. It is important to emphasize here that the discovery of refactoring \eo{s} is still important and a prerequisite for this filtering.
}{}{}


\subsection{Results}

\begin{table}[b!]
\centering
%\parbox{.45\linewidth}{
\caption{The MAP@k scores for results of Experiment 1.}
%\begin{adjustbox}{center}
\begin{tabular}{r|c c c c}
\toprule
   & \textbf{MAP@1} & \textbf{MAP@5} & \textbf{MAP@10} & \textbf{MAP@$\infty$}  \\
   \midrule
     \textbf{Compression} & \cellcolor[gray]{0.9}$0.967$ & \cellcolor[gray]{0.9}$0.974$ & \cellcolor[gray]{0.9}$0.975$ & \cellcolor[gray]{0.9}$0.975$   \\
      \textbf{Frequency}   & $0.016$ & $0.353$ & $0.368$ & $0.368$   \\
      \bottomrule
    \end{tabular}
%   \end{adjustbox}
\label{tbl:exp1_mapatk}
\end{table}
%}
%\hfill
%\parbox{.48\linewidth}{
\begin{table}[b!]
\caption{The MAP@k scores for Experiment 2.}
\centering

\begin{tabular}{r|c c c c}
\toprule
   & \textbf{MAP@2} & \textbf{MAP@5} & \textbf{MAP@10} & \textbf{MAP@$\infty$}  \\
   \midrule
     \textbf{Compression} & \cellcolor[gray]{0.9}$0.955$ &  \cellcolor[gray]{0.9}$0.969$ &  \cellcolor[gray]{0.9}$0.969$  &  \cellcolor[gray]{0.9}$0.969$   \\
      \textbf{Frequency}   & $0.013$ & $0.127$ & $0.152$ & $0.190$  \\
      \bottomrule
    \end{tabular}
\label{tbl:exp2_mapatk}
%}
\end{table}

\begin{table}[ht]
\centering
%\parbox{.45\linewidth}{
\caption{Spearman correlations for Experiment 1.}
    \begin{tabular}{r|c c c c c}
    \toprule
    & & & & & \textbf{Mean} \\
    & \textbf{p} & \textbf{Mining} & \textbf{e}  & \textbf{d} &\textbf{\#Nodes} \\
    & & \textbf{time}  &  &  &\textbf{per comp} \\
    \midrule
    \textbf{AP} & \cellcolor[gray]{0.95}$-0.07$ & \cellcolor[gray]{0.97}$-0.24$ & \cellcolor[gray]{0.97}$-0.23$ & \cellcolor[gray]{0.75}$0.12$ &  \cellcolor[gray]{0.96}$-0.21$      \\
    \textbf{AP (for $\mathbf{e>80}$)} & \cellcolor[gray]{0.97}$-0.14$ & \cellcolor[gray]{0.95}$-0.19$ & \cellcolor[gray]{0.95}$-0.19$ & \cellcolor[gray]{0.70}$0.25$ &  \cellcolor[gray]{0.88}$-0.03$      \\
    \textbf{Mining Time} & \cellcolor[gray]{0.80}$\ \ \,0.12$ & -- & \cellcolor[gray]{0.60}$\ \ \,0.89$ & \cellcolor[gray]{0.68}$0.26$ &  \cellcolor[gray]{0.62}$\ \ \,0.83$      \\
    \bottomrule
    \end{tabular}
			\label{tbl:exp1_corr}
\end{table}
%}
%\hfill
%\parbox{.5\linewidth}{
\begin{table}[ht]
\centering
\caption{The Spearman correlation matrix for Experiment 2.}

    \begin{tabular}{r|c c c c c}
    \toprule
    &  &  && & \textbf{Mean } \\
    & \textbf{p} & \textbf{Size at} &  \textbf{Mining}  & \textbf{e}  & \textbf{\#Nodes} \\
    & & \textbf{threshold} & \textbf{time} &  & \textbf{per comp} \\
    \midrule
    \textbf{AP} & \cellcolor[gray]{0.95}$-0.31$ & \cellcolor[gray]{0.85}$-0.05$ & \cellcolor[gray]{0.95}$-0.25$ & \cellcolor[gray]{0.88}$-0.07$ & \cellcolor[gray]{0.9}$-0.19$      \\
    \textbf{p} & -- & \cellcolor[gray]{0.78}$\ \ \,0.20$ & \cellcolor[gray]{0.78}$\ \ \,0.27$ & \cellcolor[gray]{0.85}$0$ & \cellcolor[gray]{0.78}$\ \ \,0.30$   \\
    \textbf{Size at Threshold}  & -- & -- & \cellcolor[gray]{0.78}$\ \ \,0.53$ & \cellcolor[gray]{0.78}$\ \ \,0.51$ & \cellcolor[gray]{0.78}$\ \ \,0.58$    \\
    \textbf{Mining Time} & -- & -- & -- & \cellcolor[gray]{0.7}$\ \ \,0.87$ & \cellcolor[gray]{0.7}$\ \ \,0.92$   \\
    \textbf{e} & -- & -- & -- & -- & \cellcolor[gray]{0.7}$\ \ \,0.92$    \\
    \bottomrule
    \end{tabular}
\label{tbl:exp2_corr}
%}
\end{table}

\textbf{Experiment 1:}
In Table \ref{tbl:exp1_mapatk}, we list the MAP@k scores for all datasets in the experiment. 
% \begin{table}[]
% \begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% d & p & e=1 & 5 & 10 & 25 & 50 & 75 & 90 & 95 & 100 \\ \hline
%  & 0.1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.2 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.3 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA \\ \cline{2-11} 
%  & 0.4 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{FFFFC7}2 \\ \cline{2-11} 
%  & 0.5 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.6 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & 1 & \cellcolor[HTML]{F8A102}NA \\ \cline{2-11} 
%  & 0.7 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{FFFFC7}2 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.8 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.9 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & 1 & \cellcolor[HTML]{F8A102}NA \\ \cline{2-11} 
% \multirow{-10}{*}{10} & 1.0 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & 1 & \cellcolor[HTML]{F8A102}NA \\ \hline
%  & 0.1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{FFCE93}78 \\ \cline{2-11} 
%  & 0.2 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.3 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.4 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.5 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.6 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{FFFC9E}3 & 1 & 1 \\ \cline{2-11} 
%  & 0.7 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \cline{2-11} 
%  & 0.8 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{FFFFC7}2 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & 1 \\ \cline{2-11} 
%  & 0.9 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & 1 & 1 \\ \cline{2-11} 
% \multirow{-10}{*}{20} & 1.0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{F8A102}NA & \cellcolor[HTML]{FFFC9E}4 \\ \hline
% \end{tabular}
% \caption{The rank of the edit operation versus the independent parameters. NA means that the correct edit operation has not been found or pruned.}
% \label{tbl:exp1_ranks}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=0.8\columnwidth, trim= 40 40 20 20, clip]{pics/spearman_exp1.png}
% 			\caption{Spearman corrleations for the first experiment.}
% 			\label{fig:exp1_corr}
% \vspace{-1em}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In table \ref{tbl:exp1_ranks}, we list the rank of the \eo{} depending on our control parameters $d$, $e$ and $p$. 
Table \ref{tbl:exp1_corr} shows the Spearman correlation of the independent and dependent variables. If we look only on datasets with a large number of applied \eo{s}, $e > 80$, the Spearman correlation for average precision vs. $d$ and average precision vs. $p$ becomes $0.25$ (instead of $0.12$) and $-0.14$ (instead of $-0.07$), respectively.
The mean time for running \textsc{Gaston} on our datasets was 1.17s per dataset.

%For our algorithm, we have to set the support threshold $t$ and the maximal number of nodes in our graphs.
%Depending on these parameters, we then investigate the rank of the correct \eo{} in the output of the algorithm and the total running time.

% \begin{figure}[ht]
% 			\centering
% 			\includegraphics[width=0.6\columnwidth]{pics/eos_vs_components.png}
% 			\caption{Adding more \eo{s} to the difference eventually leads to decreasing number of components.}
% 			\label{fig:eos_vs_components}
% \end{figure}

\textbf{Experiment 2:}
In Table \ref{tbl:exp2_mapatk} we give the MAP@k scores for this experiment. Table \ref{tbl:exp2_corr} shows the correlation matrix for the second experiment. The mean time for running \textsc{GASTON} on our datasets was 1.02s per dataset.

\textbf{Experiment 3:}
Table \ref{tbl:exp3-stats} shows the results for the Likert values for the mined and random \eo{s} for the five participants of our study. Furthermore, we conduct a t-test and a Wilcoxon signed-rank test, to test if the mined \eo{s} more likely present typical edit scenarios than the random ones. The p-values are reported in Table \ref{tbl:exp3-stats}.

\textbf{Null hypothesis $\mathbf{H_0}$:} \textit{The mined \eo{s} do not present a more typical edit scenario than random \eo{s} on average.}\par

We set the significance level to $\alpha = 0.01$.  We can see that, for all participants, the mean Likert score for the mined operations is significantly higher than the mean for the random operations. We can therefore reject the null hypothesis.

\begin{table}[htbp]
\centering
\caption{Statistics for the Likert values for Experiment 3.}
\begin{tabular}{$c^c^c^l^l}
\toprule
\rowstyle{\bfseries} Participant & Mean & Mean & p-value & p-value\\
\rowstyle{\bfseries} & mined & random & (t-test) & (Wilcoxon)\\
\midrule
P1          & $3.20$       & $1.68$        & $11.8\cdot10^{-5}$  & $29.0\cdot10^{-5}$  \\
P2          & $4.04$       & $2.76$        & $16.6\cdot10^{-4}$ & $6.43\cdot10^{-3}$ \\
P3          & $4.32$       & $2.60$        & $9.30\cdot10^{-6}$ & $5.87\cdot10^{-5}$  \\
P4          & $4.32$       & $1.08$        & $2.67\cdot10^{-15}$ & $3.51\cdot10^{-10}$ \\
P5          & $4.48$       & $1.60$        & $1.17\cdot10^{-11}$ & $1.15\cdot10^{-7}$ \\
\midrule
\textbf{Total} & $\mathbf{4.072}$ & $\mathbf{1.944}$  & $\mathbf{<2.2\cdot10^{-16}}$ &  $\mathbf{<2.2\cdot10^{-16}}$\\
\bottomrule
\end{tabular}
\label{tbl:exp3-stats}
\end{table}
\inExtension{Note that we also correlated the frequency of the \eo{s} in our dataset with the average Likert value from the interviews. We found a small but insignificant correlation (Pearson correlation of $0.33$, $p=0.12$).}{}{}

After their rating, when we confronted the engineers with the true results, they stated that the \eo{s} obtained by \textsc{Ockham} represent typical edit scenarios. According to one of the engineers, some of the \eo{s} ``can be slightly extended'' (see also \secref{sec:discussion}). Some of the \eo{s} found by \textsc{Ockham}, but not recognized by the participants, where identified ``to be a one-off refactoring that has been performed some time ago''.\par
\changed{In this real-world repository, we found some operations that are typical to the modeling language SysML, for example, one which is similar to the simplified operation in Figure \ref{fig:approach}. We also found more interesting operations, for example, the addition of ports with domain-specific port properties. Furthermore, we were able to detect some rather trivial changes. For example, we can see that typically more than just one swimlane is added to an activity, if any. We also found simple refactorings, such as renaming a package (which also leads to changing the fully qualified name of all contained elements) or also refactorings that correspond to changed conventions, for example, activities were owned by so called {\sf System Use Cases} before but have been moved into {\sf Packages}.}

\inExtension{
\textbf{Experiment 4:}
%%%%%%%%%%%%%%%%%
When performing the semantic lifting with the 30 selected \eo{s} on the 40 model differences, we first observe that we matched only $30\%$ of the total changes in our model differences. Furthermore, with respect to our classification of the \eo{s} in noncritical and critical \eo{s}, we observe that noncritical \eo{s} occur more than twice as often as critical \eo{s}. We had $13,870$ occurrences, on average, for a noncritical \eo{} and $6,027$ occurrences for a critical \eo{}.\par
%%%%%%%%%%%%%%%%%%%
In Table \ref{tbl:exp4-stats}, we report the number of changes before the semantic lifting, the number of changes after lifting (i.e., changes not covered by any change set plus the number of change sets), the number of ``unlifted changes'' (i.e., changes not covered by any change set), the relative compression $\operatorname{c_{rel}}$, and the total compression $\operatorname{c}$. 
Our sample of 40 model differences consists of $\sim1.3$  million changes.
With the exception of one \eo{}, we found all \eo{s} in our samples. On average an \eo{} has $8,189$ occurrences in the dataset. 
We report these values for all 40 model differences together (referred to as ``Total'' in Table \ref{tbl:exp4-stats}), for the average over the 40 model differences (referred to as ``Average'' in Table \ref{tbl:exp4-stats}), their standard deviation (referred to as ``Std. Dev.'' in Table \ref{tbl:exp4-stats}), the minimum, and the maximum over the 40 model differences . Furthermore, we also report the compression ratios for the case where we restricted the semantic lifting to the set of critical edit operations. \par
We observe a relative compression ratio $\operatorname{c_{rel}}$ (see definition above) of $4.00$ over all 40 model differences.
In contrast, the total compression ratio $\operatorname{c}$ is $1.29$. When restricting the set of \eo{s} in the semantic lifting to the set of critical \eo{s}, we achieve a relative compression  ratio $\operatorname{c_{rel}}$ of $5.88$. Since we are considering a smaller set of \eo{s} for the lifting in this case, the total compression ratio for our critical \eo{s} is smaller.\par

\begin{table}[htb]
\centering
\caption{Statistics for the semantic lifting.}
\small
\begin{tabular}{c|lllll}
\toprule
\vtop{\hbox{\strut }\hbox{\strut }} & \vtop{\hbox{\strut Total}\hbox{\strut Changes}} &  \vtop{\hbox{\strut Changes }\hbox{\strut Lifted}} & \vtop{\hbox{\strut Unlifted}\hbox{Changes}} & \vtop{\hbox{\strut Relative}\hbox{Compr.}}              & \vtop{\hbox{\strut Total}\hbox{\strut Compr.}}              \\
\midrule
\textbf{Total} & $1,302,591$          & $1,006,136$       & $907,361$        & $4.00$  & $1.29$  \\
\textbf{$\text{Total}_{Crit}$} & $1,302,591$          & $1,040,814$       & $987,194$        & $5.88$  & $1.25$  \\
\textbf{Average} & $32,564.78$ & $25,153.40$ & $22,684.03$ & $3.74$ & $1.41$\\
\textbf{Std. Dev.} & $27,321.05$ & $21,248.99$ & $19,425.70$ & $1.52$ & $0.28$\\
\textbf{Min} & $16$ & $10$ & $0$ & $1.91$ & $1.10$\\
\textbf{Max} & $73,706$ & $56,032$ & $51,500$ & $10.65$ & $2.22$\\
\bottomrule
\end{tabular}
%\footnotetext{This table shows statistics of the number of changes (before and after lifting) and compression achieved on a sample of 40 differences.}
\label{tbl:exp4-stats}
\end{table}

Another observation that can be made from the semantic lifting is that the distribution of the occurrences of \eo{s} over the model differences are rather heterogeneous (see \figref{fig:change_profiles}), even though for some of the model differences their distribution highly correlates. We elaborate on this observation in \secref{sec:addapplications}.

 \begin{figure}[ht]
 			\centering
 		    \includegraphics[width=\columnwidth]{pics/change_profiles.png}
 			\caption{This plot shows for every model difference the distribution of the \eo{s}. That is, every column is a kind of change profile for the corresponding model difference. The darker the color, the higher the (relative) frequency of the \eo{} in this model difference.}
 			\label{fig:change_profiles}
 \end{figure}

}{}{}

==> Content/intro_eo_original.tex <==
\section{Introduction}
Software and systems become increasingly complex. Various languages, methodologies, and paradigms have been developed to tackle this complexity.
One widely-used methodology is model-driven engineering (MDE) \cite{RodriguesDaSilva2015}, which uses models as first class entities and facilitates generating documentation and (parts of the) source code from these models. Usually, domain-specific modeling languages are used and tailored to the specific needs of a domain. This reduces the cognitive distance between the domain experts and technical artifacts. A key ingredient of many tasks and activities in MDE are model transformations \cite{Sendall2003}. 
%A model transformation transforms one model into another model. 

We are interested in \eo{s} as an important subclass of model transformations. An \emph{edit operation} is an in-place %(i.e., within one model) 
model transformation and usually represents regular evolution \cite{visser2007model} of models. For example, when moving a method from one class to another in a class diagram, also a sequence diagram that uses the method in message calls between object lifelines needs to be adjusted accordingly. To perform this in a single edit step, one can create an \eo{} that executes the entire change, including all class and sequence diagram changes.
Some tasks can even be completely automatized and reduced to the definition of \eo{s}: Edit operations are used for model repair, quick-fix generation, auto completion~\cite{ohrndorf2021history, hegedus2011quick, Kogel2016}, model editors \cite{taentzer2007generating, ehrig2005generation},  operation-based merging \cite{koegel2009operation, schmidt2009history}, model refactoring \cite{Mokaddem2018, Arendt2013},  model optimization \cite{burdusel2018mdeoptimiser}, meta-model evolution and model co-evolution \cite{rose2014graph, arendt2010henshin, herrmannsdoerfer2010extensive, getir2018supporting, kolovos2010taming}, semantic lifting of model differences \cite{Kehrer2011, kehrer2012understanding, ben2012search, langer2013posteriori, khelladi2016detecting}, model generation \cite{pietsch2011generating}, and many more.

% In general reuse is an important point in reducing complexity. \cite{Krueger1993}  -> Does not fit into the argumentation line here.

% % Applications of model transformations
% \begin{itemize}
%     %\item Pattern detection \cite{wenzel2006model}
%     \item Repair, quick-fix generation, auto completion\cite{ohrndorf2021history, hegedus2011quick, Kogel2016}
%     \item Slicing \cite{pietsch2017incrementally}
%     \item Model editors \cite{taentzer2007generating, ehrig2005generation}
%     \item Operation-based merging \cite{koegel2009operation}
%     %\item Model checking and  smell detection \cite{Arendt2013}
%     \item Model refactoring \cite{Mokaddem2018, Arendt2013}
%     \item Model optimization \cite{burdusel2018mdeoptimiser}
%     \item Model Co-Evolution and meta-model evolution \cite{rose2014graph, arendt2010henshin, herrmannsdoerfer2010extensive}  % (Not covered by our current approach but should also be possible by extension, i.e. Meta-Model is the Meta-Meta Model in this case) 
%     \item Artifact co-evolution in general \cite{getir2018supporting, kolovos2010taming} %(e.g., EMF and GMF \cite{kolovos2010taming,})
%     \item Semantic lifting of model differences \cite{Kehrer2011, kehrer2012understanding, ben2012search, langer2013posteriori, khelladi2016detecting}
%     \item Mutation-based fuzzing \cite{nguyen2020mofuzz}
%     \item Delta-oriented development in model-based product line engineering \cite{pietsch2015sipl, seidl2014deltaecore}
%     \item Model generation \cite{pietsch2011generating}
% \end{itemize}


%``pull up attribute refactoring'', where a common attribute from child classes is moved to the parent class, can be defined as an \eo{} and then automatically be executed on the models.

%General overview of Model transformations: Further uses in \url{http://staffwww.dcs.shef.ac.uk/people/A.Simons/remodel/papers/BiehlModelTransformations.pdf} chapter 3.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Reasons for automatically learning the transformations
In general, there are two main problems involved in the specification of \eo{s} or model transformations in general.
Firstly, creating the necessary transformations for the task and the domain-specific modeling languages at hand using a dedicated transformation language requires a deep knowledge of the language's meta-model and the underlying paradigm of the transformation language. It might even be necessary to define project-specific \eo{s}, which causes a large overhead for many projects and tool providers \cite{Kehrer2017, Mokaddem2018, Kappel2012}.
Secondly, for some tasks, domain-specific transformations are a form of tacit knowledge \cite{Polanyi1958}, and it will be hard for domain experts to externalize this knowledge.
%Thirdly, the transformations can change over time, e.g., because the meta-model changes, and therefore the operations would have to be maintained. 

% Short related-work and motivation
As, on the one hand, model transformations play such a central role in MDE, but, on the other hand, it is not easy to specify them, attempts have been made to support their manual creation or even (semi\nobreakdash-)automated generation.
%For example, there are approaches that generate model transformations out of the meta-model \cite{Kehrer2016, mazanek2009generating}, from a given set of positive (and negative) application examples \cite{Varro2006, Kehrer2017, Baki2016, Mokaddem2018, faunes2013genetic}, operation recorders \cite{Langer2009, Gray2011, Kappel2012}, or visual assistance tools \cite{Avazpour2015}.
As for manual support, visual assistance tools \cite{Avazpour2015} and transformation languages derived from a modeling language's concrete syntax \cite{acrectoaie2018vmtl, holldobler2015systematically}  have been proposed to release domain experts from the need of stepping into the details of meta-models and model transformation languages. However, they still need to deal with the syntax and semantics of certain change annotations, and edit operations must be specified in a manual fashion.
To this end, generating edit operations automatically from a given meta-model has been proposed \cite{Kehrer2016, mazanek2009generating, kehrer2013generating}. However, besides elementary consistency constraints and basic well-formedness rules, meta-models do not convey any domain-specific information on \emph{how} models are edited. Thus, the generation of edit operations from a meta-model is limited to rather primitive operations as a matter of fact. 
Following the idea of model transformation by-example (MTBE) \cite{Langer2009, Gray2011, Kappel2012}, initial sketches of more complex and domain-specific edit operations can be specified using standard model editors. However, these sketches require manual post-processing to be turned into general specifications, mainly because an initial specification is derived from only a single transformation example.
Some MTBE approaches \cite{Kehrer2017, Mokaddem2018} aim at getting rid of this limitation by using a set of transformation examples as input, which are then generalized into a model transformation rule. Still, this is a \emph{supervised} approach, which requires sets of dedicated transformation examples that need to be defined by domain experts in a manual fashion. As discussed by \cite{Kehrer2017}, a particular challenge is that domain experts need to have, at least, some basic knowledge on the internal processing of the MTBE tool to come up with a reasonable set of examples. Moreover, if only a few examples are used as input for learning, \cite{Mokaddem2018} discuss how critical it is to carefully select and design these examples. 

%[3,9,28, und auch noch weitere...] address the larning of exogenous out-place model-2-model transformations. Inwiefern wir sie hier überhaupt erwähnen sollen hängt davon ab, wie früh wir auf das spezielle Anwendungsszenario in-place transformations / edit operations zusteuern.


%Edit operations as e special form of model transformations
% In this work, we focus on a \eo{s} as a special kind of model transformations. Most of the existing approaches for this kind of operation are based on a concrete set of examples and therefore the transformations will only be as good as the given examples. Indeed, you kind of need to know what the tools are doing in order to present good examples. 
% \textcolor{red}{
% (TODO Timo Kehrer -> Can you provide some proof/reference for this statement?)
% }
% Other approaches, e.g., generating transformations out of the meta-model, are not able to create complex \eo{} but rather ``trivial'' ones. 

% Our approach
To address these limitations of existing approaches, we propose a novel \emph{unsupervised} approach, \textsc{Ockham}, for mining \eo{s} from existing models in a model repository, which is typically available in large-scale modeling projects (cf.~\secref{sec:case-study}). \textsc{Ockham} is based on an Occam's razor argument, that is, the \emph{useful} \eo{s} are the ones that \emph{compress} the model repository. In a first step, \textsc{Ockham} discovers frequent change patterns using \emph{frequent subgraph mining} on a labeled graph representation of model differences. It then uses a \emph{compression metric} to filter and rank these patterns. We evaluate \textsc{Ockham} using two controlled experiments with simulated data and one real-world large-scale industrial case study from the railway domain. In the controlled setting, we can show that \textsc{Ockham} is able to discover the \eo{s} that have been actually applied before by us, even when we apply some perturbation. In the real-world case study, we find that our approach is able to scale to real-world model repositories and to derive \eo{s} deemed reasonable by practitioners. We evaluated \textsc{Ockham} by comparing the results to randomly generated \eo{s} in five interviews with practitioners of the product line. We find that the \eo{s} represent typical edit scenarios and are meaningful to the practitioners. \inExtension{Additionally, we evaluate the practical applicability of the derived \eo{s} based on a concrete real-world scenario.}{}{}

In a summary, we make the following contributions:
\begin{itemize}
    \item We propose an unsupervised approach, called \textsc{Ockham}, that is based on frequent subgraph mining to derive \eo{s} from model repositories, without requiring any further information.
    \item We evaluate \textsc{Ockham} empirically based on two controlled simulated experiments and show that the approach is able to discover the applied \eo{s}.
%    \item We describe a MDE challenge in a real-world project and how \eo{s} can be used to mitigate the challenge.
    \item We evaluate the approach using an interview with five experienced system engineers and architects from a real-world industrial setting in the railway domain with more than 200 engineers, 300GB of artifacts, and more than 6 years of modeling history. We show that our approach is able to detect meaningful \eo{s} in this industrial setting and that it scales to real-world repositories.
    \inExtension{
    \item We apply the automatically derived \eo{s} in the concrete use case of condensing large model differences and show their practical impact in this case. We furthermore argue how the \eo{s} can be used to analyze and simulate model evolution.  
    }{}{}
\end{itemize}

\inExtension{
This article is an extension of a conference paper published at ASE'21~\cite{Tinnes2021}. In the conference version, we presented and evaluated \textsc{Ockham}, an unsupervised learning approach for mining domain-specific \eo{s} from model histories. In this article, we include two major additions. First, we evaluate the practical implications of the obtained \eo{s} using a real-world case study. More specifically, motivated by our aim to facilitate the analysis of model differences, we evaluate the extent to which the \eo{s} can be used to compress and filter model differences. Second, we discuss key observations that we made in the case study when further analyzing model differences after a semantic lifting using the \eo{s} mined by \textsc{Ockham}. In particular, we have found that the frequency distribution of the edit operations in the model differences gives rise to a change profile that describes the model difference from a statistical perspective and can be used for classifying the model differences. We discuss applications of these profiles, including the statistical analysis of model differences and the use of the change profiles to simulate model evolution.
}{}{}

==> Content/intro_meta.tex <==
\todo[inline]{Aktuell kann ich leider nicht ``überzeugend'' zeigen, dass der Sprachmodell (LM) Ansatz zum Mining von Modelltransformationen klare Vorteile gegenüber dem Frequent Subgraph Mining (FSM) basierten Ansatz hat. Ich kann natürlich Parameter im FSM so finden, dass FSM auf die Nase fliegt, während der LM Ansatz noch brauchbare Ergebnisse liefert. Ich würde sagen, dass für Mining von Modelltransformationen per Sprachmodell die Forschung noch in einem zu frühen Stadium ist (für die Erwartungen der SE Community). Einen großen Vorteil sehe ich aber \emph{jetzt schon} darin, dass ich mit dem Sprachmodell generell auch kontextabhängige Modellvervollständigungen machen kann. Für das Paper würde ich daher gerne diesen Punkt auch ausspielen. Ich denke, das erhöht die Annahmechancen deutlich. Daher habe ich mir überlegt, wie ich Modellvervollständiungen auch aus der Brille von Editieroperationen sehen kann. Die Idee ist, von \emph{dynamischen Editieroperationen oder Completion Operations} zu sprechen. Eine Vervollständigung liefert quasi automatisch eine Modelltransformation (da wir auf Änderungsgraphen arbeiten). Diese ist abhängig von der ``angefangenen Änderung'' und (optional/perspektivisch) dem kompletten Kontext. Was Vervollständigungen angeht, performen die Modelle tatsächlich sehr gut, wobei das finale Experiment noch aussteht.}
Story/Motivation: 
\begin{itemize}
    \item Model evolution is important
    \item We can see model evolution as edit operations acting on the models
    \item Side note: Edit Operations can be seen as model transformation which play a very important role in MDE (list some new cases, e.g., realistic simulation here)
    \item Modelling tools typically provide initial sets of EOs, but it's hard to define further (implicit) ones because of abstract language for their definition and the fact that they often are tacit knowledge
    \item MTBE (model-transformation-by-example) has been proposed but it turned out that engineers need to know tool internals to come up with good examples (therefore failed)
    \item Edit Operation Mining has been introduced (our work), but is not scalable at not flexibel enough. Especially large "completions" might be interesting. Also context awareness might be interesting. For the shortcomings see Table \ref{tbl:shortcomings}.

    \begin{table*}[]
        \centering
        \begin{tabular}{l l l l }
                \toprule
                \textbf{Property} & \textbf{FSM} & \textbf{Language Model} & \textbf{Research} \\
                                &     &  & \textbf{Question/Experiment} \\
                \midrule
             Completions ("dynamic EO") & Context to specific & ``solved'' & RQ1\\
             Abstraction (e.g., Inheritance) & no solution & \textbf{interesting question!} & No Data yet, probably "ad-hoc"??\\
             Scalability & No & Kind of solved, but hard to compare & TBD (e.g., arguing via pricing?)\\
             Correct Graph and Type & Always & Not necessarily & RQ2\\
             Memorization vs. Understanding & Memo only & Understanding & RQ4\\
             EO Readout & Compression & Sampling + Metric? & RQ3, RQ5\\
             Connectivity & connected only & unconnected possible\footnote{Therefore overcoming the limitations of SCGs} & No Data yet (TBD?) \\
             Derive Attribute Relationship & Not part of the approach & Could be learned & No data yet (TBD?)\\
                \bottomrule
        \end{tabular}
        \caption{Shortcomings of \textsc{OCKHAM} that we want to discuss in this paper}
        \label{tbl:shortcomings}
    \end{table*}

    \item Motivated by recent breakthroughs (copilot, molecular generation,.. ) we propose language models to overcome some challenges 
    \item We present an language model-based approach, conduct experiments, and report on results 
\end{itemize}

Related Work:
\begin{itemize}
    \item MTBE Literature
    \item NLP in model driven engineering
    \item NLP for model transformation learning (there is a research strand by Loli Burgueño, but they are supervised... probably should get in touch anyway)
    \item Pattern Mining and Program Synthesis (FlashMeta ...)
    \item Completion Literature (incl. Model Completion)
        Completion in SE
    \item Generative Model Literature (background)
        Use cases Fuzzing and Completion and ? 
    \item Language Models (background)
        N-gram, LSTM, transformers, GPT-2-3, Codex, Github Co-Pilot, They can learn representations such as AST
\end{itemize}

Approach:
\begin{itemize}
    \item Serialize Model Difference (argue why differences are better)
    \item Train Context-Completion pairs (using pre-trained model)
    \item Completion $\rightarrow$ Easy
    \item Sampling EOS  $\rightarrow$ Need a special sampling procedure
\end{itemize}

Research Questions:

Methodology: To verify if \approach{} can help to provide model completions and  discover edit operations, we ask the following research questions:

\begin{itemize}
    \item RQ1:  Are language models capable of providing correct completions for models?
    + dependence on base model, epochs, and repo properties
    \item RQ2: Is the GRAPH syntax of the generated tokens correct? 
    + dependence on base model, epochs, and repo properties
    \item RQ3: Can edit operations be read out from the language model?
    RQ3.1: Without context.
    RQ3.2: With context
    + dependence on base model, epochs, and repo properties
    \item RQ4: Are the edit operations only memorized by the model as textual strings or is the model able to learn the underlying mechanisms (esp. graph isomorphism)
    + dependence on base model, epochs, and repo properties
    \item RQ5: Best ranking metrics, factorial weighted, edge count weighted,,, + recompute actual compression!!!
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%% FULL TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\todo[inline]{BEGIN FULLTEXT:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Content/related_original.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}

\begin{itemize}
    \item MTBE Literature
    \item Pattern Mining Literature
    \item Completion Literature (incl. Model Completion)
        Completion in SE
    \item Generative Model Literature (background)
        Use cases Fuzzing and Completion and ? 
    \item Language Models (background)
        N-gram, LSTM, transformers, GPT-2-3, Codex, Github Co-Pilot, They can learn representations such as AST
\end{itemize}


Related Work:

ANN for MTL https://ieeexplore.ieee.org/abstract/document/8906971/ (exogeneous transformations (supervised))

Also from the same authors: https://link.springer.com/article/10.1007/s10270-021-00893-y
Probably very close but supervised... Anyway, we should get in touch.

RL based Model Transformation (for optimization): https://ieeexplore.ieee.org/document/9592463/



Interpreting Language Models Through Knowledge Graph Extraction: https://arxiv.org/pdf/2111.08546.pdf


Graph-to-text generation: https://arxiv.org/pdf/2007.08426
Neural language modeling for contextualized temporal graph generation: https://arxiv.org/pdf/2010.10077

Incorporating Domain Knowledge Into Language Models by Using Graph Convolutional Networks for Assessing Semantic Textual Similarity: Model Development and Performance Comparison: https://medinform.jmir.org/2021/11/e23101

Language Models compared to Genetic Programming for SE Tasks: https://arxiv.org/abs/2111.07875


Learning functional properties of proteins with language models: https://www.nature.com/articles/s42256-022-00457-9.pdf 


What Do They Capture? - A Structural Analysis of Pre-Trained Language Models for Source Code:
https://arxiv.org/pdf/2202.06840.pdf
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9616462

Models/Graphs:
Motif Generation via LM in Bio-/Chemical Datasets: https://project-archive.inf.ed.ac.uk/ug4/20212351/ug4_proj.pdf

Search String (to be refined):
("pretraining" | "pre-training" | "transfer learning" | "transformer" | "deep learning") ("model completion" | "model transformation" | "edit operation") ( "uml models" | "eclipse modeling framework" |  "Simulink" | "SysML" | "IEC 61131-3")
First 11 pages

(~"language models" OR GPT-3) AND ("motive" OR "graph pattern" OR "graph motif" OR "motif" OR "subgraph")

"Pretraining for EMF/uml/Simulink"

Simulink GPT-2 Generation:
https://ranger.uta.edu/~csallner/papers/Shrestha21SLGPT.pdf
An NLP-based architecture for the autocompletion of partial domain models
https://hal.archives-ouvertes.fr/hal-03010872/file/Domain_Model_Autocompletion.pdf
https://modeling-languages.com/wp-content/uploads/2019/07/Sosym_Neural_Networks_for_Model_Manipulation_preprint.pdf
https://arxiv.org/pdf/2104.01642.pdf


Datasets:
https://link.springer.com/content/pdf/10.1007/s10270-021-00883-0.pdf






% In PhD Thesis, also compare to model repair (see ohrndorf), model evolution (<- Extra paper), ...

\changed{Various approaches have been proposed to (semi-)automatically learn model transformations in the field of model transformation by example (MTBE).
%there are approaches that derive operations from the meta-model \cite{Kehrer2016, mazanek2009generating}, others rely on an operation recorder \cite{Langer2009, Gray2011, Kappel2012} and mining techniques can be used to derive further complex operations \cite{Kogel2016} and some propose to learn the model transformations from a set of given examples \cite{Kehrer2017, Mokaddem2018}. Operation recording and learning operations from a set of given examples is usually referred to as model transformation by-example (MTBE). Since we are interested in learning \eo{s}, we focus here on endogenous (i.e., source and target meta-model are equal) model transformations.
%We furthermore performed an informal literature review to be able to better put our case study into perspective of existing challenges in the area of model evolution and \sple{}. During our literature review, we did not find any research that is tackling the problems with a \cao{} approach to \sple{} in a practical setting. Some of the difficulties and challenges are mentioned by the research community, but research about how to overcome the challenges without starting from scratch and with the given constraints in an industrial setting is rare. 
% \subsection{Model Transformation \mbox{by-Example}}
%Even though some of the available tools allow for a visual, declarative definition of model transformations it is usually still a time-consuming activity and demands for the knowledge of another language that is not directly linked to the language the modeller is using.
%For example, \textsc{Henshin} rules are based on the abstract syntax but tool users are more familiar with the concrete syntax of their models. 
% I think this should be kind of obvious but if sources are needed, "MTBE: A survey of the first wave" mentions some references. But in Thesis also give an introduction into concrete vs. abstract syntax. The edit operations as we understand them are more like (possibly hidden) concepts. As such they have to be compared to concrete syntax and also Kehrers effective MMs. I think, in the end, these are all ways for efficient handling of concept hiding. 
%Therefore approaches have been proposed to learn model transformations from examples, so called \textit{model transformation by-example} (MTBE). It's important to distinguish here between exogenous, i.e., model and transformed model conform to a different meta-model, and endogenous model transformations, i.e., the models conform to the same meta-model.
%TODO add "From Examples to Knowledge in Model-Driven Engineering: a Holistic and Pragmatic Approach" as an important consideration how to derive good examples for learning.
In the first systematic approach of MTBE, \cite{Varro2006} proposes an iterative procedure that attempts to derive {\em exogenous} (i.e., source and target meta-model are different) model transformations by examples. Appropriate examples need to be provided for the algorithm to work.
Many approaches to learning exogenous model transformations have been proposed until now. For example,  \cite{berramla2020} use statistical machine translation and language models to derive transformations. \cite{Baki2016} apply simulated annealing to learn operations. 
%Note that the search space typically becomes huge when the transformations are learned in an unsupervised manner which is possibly why more and more meta-heuristic MTBE approaches are emerging.
Regarding \emph{exogenous} transformations there is also an approach by \cite{Saada2014}, which uses graph mining techniques to learn concepts, which are then used to identify new transformation patterns. %Contrary to our approach, they also apply the graph mining to a set of concrete examples.
}
% Note that for exogenous transformations also saada et al. Learning model transformation patterns using graph generalization apply FSM to extract the "examples" from the whole set of data

\changed{As mentioned in the introduction, most closely related approach to ours is MTBE for {\em endogenous} model transformations.}
Compared to exogenous MTBE, there are only a few studies available for endogenous MTBE. \cite{Langer2009} present a tool called \textsc{Operation Recorder}, which is a semi-automatic approach to derive model transformations by recording all transformation steps. A similar approach is presented by \cite{Gray2011}, who also infer complex model transformations from a demonstration. \cite{Jalali2012} learn transformation rules from a set of examples by generalizing over pre- and postcondition graphs. Their approach has been applied to the derivation of \eo{s}, including negative application conditions and multi-object patterns by \cite{Kehrer2017}. 
Instead of learning a single operation, \cite{Mokaddem2018} use a genetic algorithm to learn a set of refactoring rule pairs of examples before and after applying refactorings. The creation of candidate transformations that conform to the meta-model relies on a ``fragment type graph'', which allows them to grow candidate patterns that conform to the meta-model. % similar to the pattern growth algorithms in FSM but additionally they conform to the meta-model. 
Their algorithm optimizes a model modification and preservation score. \cite{Ghannem2018} also use a genetic algorithm (i.e., NSGA-II) to learn model refactorings from a set of ``bad designed'' and ``good designed'' models. Their approach  distinguishes between structural similarity and semantic similarity and tries to minimize structural and semantic similarity between the initial model and the bad designed models and to maximize the similarity between the initial and the well designed models.
\par

%\begin{remark}
%There are also approaches that create the \eo{s} from the meta-model. For instance, Kehrer et al. \cite{Kehrer2016} generate consistency preserving \eo{s} from the meta-model. These \eo{s} are minimal in the sense that every smaller operation might break the consistency of the model.
%\end{remark}

All of these approaches for learning endogenous model transformations are (semi-)supervised. Either a concrete example is given (which only contains the transformation to be learned) or a set of positive and negative examples is given. In the case of Mokaddem et al.'s genetic approach, it is assumed that all transformations that can be applied are actually applied to the source models. 
For the meta-model used in our real-world case study, we do not have any labeled data. In general, we are not aware of any fully unsupervised approach to learn endogenous model transformations. To reduce the search space, we leverage the evolution of the models in the model repository, though. We do not directly work on the models as in the approaches discussed above, but we work on structural model differences. \par

% Pattern mining and discovering meaningful differences in code
\changed{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Related work in source code%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Furthermore, there is related work in the source code domain.
%%%%Code - Filtering and Pattern Detection%%%%
Regarding one of our motivations for mining \eo{s}, namely to simplify differences, there are several approaches in the source code domain \citep{Yu2011, martinez2013}. %where a user can define a program normalization which is used in combination with clone detection to detect meaningful changes in the differences between program revisions. Meaningful changes in their work are defined by a developer. 
These approaches are more comparable to the approach of semantic lifting \citep{Kehrer2011}, to aggregate or filter model differences according to given patterns but they are not learning the patterns themselves.
%Martinez et al. \cite{martinez2013} propose an AST-based approach to identify instances of code change patterns but the patterns have to be defined by hand. The approach is applied to analyze the version history of Java software projects. 
%In contrast, we automatically group low level changes to meaningful changes, i.e., changes that typically belong together are grouped together in the model differences. We could classify certain high-level changes as meaningful or irrelevant in the semantic lifting \cite{Kehrer2011} to filter the model differences accordingly. 
%%%%Code - Pattern Mining%%%%
There are also approaches to mine change patterns in source code. For example, \cite{Dagit2013} propose an approach based on the abstract syntax tree, and \cite{nguyen2019} mine patterns based on a so called fine-grained program dependence graph. \inExtension{\cite{janke2020} derive \emph{fine-grained edit scripts} from abstract syntax tree differences and transform them to a graph representation for graph mining.}{}{} %propose an algorithm to identify source code change patterns by grouping changes in the abstract syntax tree (AST) and generalizing these groups by performing some anti-unification.  %The main difference is that Dagit et al. work on trees whereas \textsc{Ockham} works on a kind of abstract syntax graphs which already include domain knowledge given by the meta-model. 
%A more recent code change pattern mining algorithm is given by Nguyen et al. \cite{nguyen2019} which does not operate on the AST but on a so called fine-grained program dependence graph. They don't use generic (frequent) subgraph miners but propose their own approximation algorithm which utilizes knowledge about the change patterns and a clone detection technique for clustering. 
There is also some work that focuses on mining design patterns from source code~\citep{Oruc2016, balanyi2003mining, ferenc2005design, dong2009review}.
%%%%Code - Differences%%%%
The idea behind these approaches --- learning (change) patterns from a version history --- is comparable to ours. In contrast to these approaches, \textsc{Ockham} works on a kind of abstract syntax graph, which already includes domain knowledge given by the meta-model. 
%This can also be understood as background knowledge we can provide to the pattern mining, that is, there is no need to work on higher levels of abstraction, as, for example in our case, the M0-level of the Meta-Object Facility \cite{omg2013mof}.
Furthermore, we do not use a similarity metric to detect change groups or frequent changes but use an (exact) subgraph mining approach. In model-driven engineering, one often has some kind of identifiers for the model elements, which makes the differencing more reliable and removes the need for similarity-based differencing methods. }


